Correcting Two Deletions and Insertions in Racetrack Memory

Racetrack memory is a non-volatile memory engineered to provide both high density and low latency, that is subject to synchronization or shift errors. This paper describes a fast coding solution, in which delimiter bits assist in identifying the type of shift error, and easily implementable graph-based codes are used to correct the error, once identified. A code that is able to detect and correct double shift errors is described in detail.

==> Beyond.tex <==
In Section~\ref{Section:Racetrack}, we assumed that in every $m-1$ shifts at most one shift error may occur. In this section, we take the first steps in relaxing this assumption and we discuss the challenges that arise by doing so. In particular, we assume the memory behaves {\it mostly} in accordance with the assumption stated above. However, occasionally a combination of one deletion and one repetition may occur within $m-1$ shifts. Moreover, if we have one deletion and one repetition in $m-1$ consecutive shifts, then we do not see another shift error for at least $2(m-1)$ following shifts. This latter assumption is to guarantee proper error detection. 

We first need to describe how to detect a combination of one deletion and one repetition. We then use an outer-code on top of the code presented in Section~\ref{Section:Practical} to correct such errors. We have the following result for VT codes.
\begin{lemma}
\label{Lemma:combination}
For any two binary strings  $\mathbf{x}, \mathbf{y} \in VT\left( n \right)$, $\mathbf{y}$ cannot be obtained from $\mathbf{x}$ by a deletion followed by an insertion (or by an insertion followed by a deletion).
\end{lemma}

\begin{proof}
Suppose $\mathbf{x}^\prime \in D_{-1}\left( \mathbf{x} \right)$ and $\mathbf{y}^\prime \in D_{-1}\left( \mathbf{y} \right)$. If $\mathbf{y}$ can be obtained from $\mathbf{x}$ by a deletion followed by an insertion, then 
\begin{align}
D_{+1}\left( \mathbf{x}^\prime \right) \cap D_{+1}\left( \mathbf{y}^\prime \right) \neq \emptyset.
\end{align}
In other words, $\mathbf{x}$ and $\mathbf{y}$ do not satisfy (\ref{Eq:CodeRequirement}). However, this contradicts Lemma~\ref{Lemma:VTGraphBased}. This contradiction proves the result. A similar argument can be used when an insertion is followed by a deletion. 
\end{proof}

Lemma~\ref{Lemma:combination} immediately results in the following observation.
\begin{corollary}
A combination of a deletion error and an insertion error on $\mathbf{x} \in VT\left( n \right)$ either results in $\mathbf{x}$ or in $\mathbf{y} \notin VT\left( n \right)$ (an invalid codeword).
\end{corollary}

To detect a combination of one deletion error and one insertion (or repetition) error, we can no longer solely rely on the delimiter bits. First assume no shift error happens within the delimiter bits. To detect a combination of errors, we need to calculate the check-sum as we read the stored bits. If the stored codeword between two sets of delimiter bits  $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ does not pass the check-sum constraint of (\ref{eq:VTCondition}), and the delimiter bits do not reveal any errors, we conclude that a combination of one deletion error and one insertion error has happened. 

Now suppose we detect a combination of one deletion error and one insertion (or repetition) error by observing an invalid codeword as described above. We can use an outer-code to recover data in this case as illustrated in Fig.~\ref{Fig:OuterCode} where the outer-code is a simple single parity code. We note that we use VT codes to correct single shift errors and to detect a combination deletion and repetition errors.

Next, we need to understand what happens if one (or two) error happens within the delimiter bits. To see why this issue requires attention, consider the delimiter bits $(100)$ and suppose the first bit is deleted and the second bit is repeated. Thus, when we read the memory we observe $000$ instead of the $100$ pattern. According to Table~\ref{Table:Syndrom}, this observation corresponds to a deletion in the first $m-3$ shifts which is not correct.
Since we assumed that no more shift errors happen for at least $2(m-1)$ shifts after a combination of deletion and repetition errors, we can identify this false detection using the next set of delimiter bits. In particular, when we observe the following $100$ pattern, we update our previous error detection accordingly. Thus, we need to wait to see the next set of delimiter bits before we attempt to recover data from the memory.

In this section, we only considered having a combination of one deletion and one repetition. Dealing with other combinations of two shift errors (\emph{e.g.}, two deletions) is more challenging. First is the issue of detection. The delimiter bits we introduced in this paper work well for detecting a single shift error and we could use them with the VT codes to detect a combination of one deletion and one repetition. However, it is not an easy task to modify them in order to detect two deletion errors or two repetition errors. Error detection for multiple shift errors is an interesting subject for future work. 

Second is the issue of correction. Conceptually we can design codes that can correct multiple shift errors. However, the encoding complexity quickly increases. Unfortunately, we are not aware of codes that similar to VT codes have reasonable encoding and decoding complexity. However, we believe exploiting the spatial diversity of racetrack technology (having multiple tracks in parallel) may enable us to correct multiple shift errors once they are detected.

==> Conclusion.tex <==
We introduced a single-shift-error-detecting (SSED) single-shift-error-correcting (SSEC) code for racetrack memory. Our code does not require any hardware modifications and has a storage overhead that is logarithmic in the length of the codeword. We separated detection from correction to make the common case in which no error happens, fast and efficient. We showed how non-linear graph-based codes are suitable for error correction in racetrack technology. We then focused on a specific subclass of such codes, namely Varshamov-Tenengolts codes, for which we introduced an encoding algorithm. Our proposed code is amenable to to fast encoding and decoding algorithms. We investigated the storage cost (rate) and the performance of our code, and quantified its performance and demonstrated its gain over linear codes.

The next steps include detection and correction of bit flip errors on top of shift errors. Moreover, we aim to design codes that can detect and correct multiple shift errors.

==> Delimiter.tex <==
In Section~\ref{Section:Detection}, we introduced delimiter bits to separate error detection from error correction, and we chose $100$ as delimiter bits. Here, we reveal the rationale for this choice. 

A brute force search shows that we cannot detect a shift error and its type (deletion vs. repetition) using fewer than three bits. Say we use three bits $a,b,$ and $c$ as delimiter bits. The top priority is to detect a shift error and its type in the first $m-3$ shifts since that would directly affect the bits stored prior to delimiter bits. We summarize the resulting observations in positions $m-2$, $m-1$ and $m$ for a shift error in the first $m-3$ shifts in Table~\ref{Table:SyndromRationale}.

\begin{table}[ht]
\begin{center}
\begin{tabular}{L|M|M|M|N}
\cline{2-4}
																				                       & position $m-2$ & position $m-1$ & position $m$ &\\[10pt] \hline
\multicolumn{1}{|L|}{no error}                                 & $a$              & $b$              & $c$      &\\[10pt] \hline
\multicolumn{1}{|L|}{$1$ deletion in the first $m-3$ shifts}   & $b$              & $c$              & {\sf X}  &\\[10pt] \hline
\multicolumn{1}{|L|}{$1$ repetition in the first $m-3$ shifts} & {\sf X}          & $a$              & $b$      &\\[10pt] \hline 
\end{tabular}
\vspace{2mm}
\caption{Resulting observations in positions $m-2$, $m-1$ and $m$ for a shift error in the first $m-3$ shifts. Symbol ${\sf X}$ can be either a zero or a one.\label{Table:SyndromRationale}}
\end{center}
\end{table}

To guarantee that a shift error and its type can be detected, it suffices to have $a \neq b$ and $a \neq c$. The reason is that $a \neq b$ makes the error-free observations different from those resulted from a deletion or a repetition. Moreover, $a \neq c$ makes the observations resulted from a deletion different from those resulted from a repetition. We chose $abc = 100$ based on the argument presented here.


==> Detection.tex <==
In this section, we introduce delimiter bits to detect a single deletion or a single repetition in every $m-1$ shifts. 

\begin{figure}[ht]
\centering
\includegraphics[width = \columnwidth]{FiguresPDF/Delimiter.pdf}
\caption{Every $m$ bits, we allocate three delimiter bits, $100$, for the purpose of error detection.\label{Fig:Delimiter}}
\end{figure}

Consider $m$ consecutive magnetic domains in racetrack memory. If no error happens, we need $m-1$ shifts to access and read the $m$ bits stored in these $m$ domains. We have the following result for detecting a single shift error every $m-1$ shifts.
\begin{claim}
We can detect a single shift error and its type (deletion vs. repetition) using three out of every $m$ magnetic domains in racetrack memory.
\end{claim}

\begin{proof}
In every $m$ magnetic domains, we set the last three to predetermined bits $1,0,$ and $0$ as shown in Fig.~\ref{Fig:Delimiter}. We refer to the ``$100$'' pattern in positions $m-2$, $m-1$ and $m$ as the ``delimiter bits.'' 


\begin{table}[ht]
\begin{center}
\begin{tabular}{L|M|M|M|}
\cline{2-4}
																				                       & position $m-2$ & position $m-1$ & position $m$ \\ \hline
\multicolumn{1}{|L|}{no error}                                 & 1              &  0             &  0           \\ \hline
\multicolumn{1}{|L|}{$1$ deletion in the first $m-3$ shifts}   & {\bf 0}        & 0              & {\sf X}      \\ \hline
\multicolumn{1}{|L|}{$1$ repetition in the first $m-3$ shifts} & {\sf X}        & {\bf 1}        & 0            \\ \hline \rowcolor{Gray}
\multicolumn{1}{|L|}{$1$ deletion in the last $2$ shifts}      & 1              & 0              & {\sf X}      \\ \hline \rowcolor{Gray}
\multicolumn{1}{|L|}{$1$ repetition in the last $2$ shifts}    & 1              & 0              & 0            \\ \hline
\end{tabular}
\vspace{2mm}
\caption{Resulting observations in positions $m-2$, $m-1$ and $m$ for all possible error combinations. \label{Table:Syndrom}}
% Symbol ${\sf X}$ can be either a zero or a one.
\end{center}
\end{table}

We summarize the resulting observations in positions $m-2$, $m-1$ and $m$ for all possible error combinations in Table~\ref{Table:Syndrom}. A deletion or a repetition in the first $m-3$ shifts (or the first $m-2$ observed bits) can be identified since the resulting observations in positions $m-2$, $m-1$, and $m$ do not match the $100$ pattern. For instance, if we observe a $0$ in position $m-2$, we know a deletion in the first $m-3$ shifts has happened.

The two shaded possibilities are more subtle. Suppose a repetition happens in the final two shifts. Then the resulting observation is $100$ which matches the error-free case. Interestingly, this is not a problem for the following reason. First we note that the data is stored only in the first $m-3$ bits and a repetition in the final two shifts does not affect that data. However, this error affects the stored data that follows. But since we assume at most one shift error every $m-1$ shifts, until the next set of delimiter bits, no other shift errors happen. As a result, the repetition error will be detected by the following delimiter bits. 
\end{proof}

We use the delimiter bits between $n$-bit codewords. We refer to a codeword plus the immediate delimiter bits as an {\it extended codeword} of length $m = n +3$.


==> Eval.tex <==
In this section, we investigate the storage cost (rate) and the performance of our code. As mentioned earlier, our code achieves a storage rate of 
\begin{align*}
R_{\text{VT}}\left( m \right) = \frac{m - \log_2(m-3) - 4}{m}.
\end{align*}
We plotted this rate for $m$ from $11$ ($2^3+3$) to $131$ ($2^7+3$) in Fig.~\ref{Fig:Rate}. This rate approaches $1$ as $m$ increases. In this figure, we also plotted the theoretical performance of the best linear code for racetrack memory. Even at moderate values of $m$, our code provides a significant gain over the linear code. For instance at $m = 35$ ($2^5 + 3$), our code has a rate of $0.743$ which corresponds to a $62.5\%$ improvement in terms of storage overhead compared to the linear code's rate ($0.457$). This gain approaches $100\%$ as $m$ increases. 

Besides rate, it is important to pay attention to the energy consumption of our scheme. HiFi~\cite{HiFi} detects and corrects a shift error by adding two extra read/write ports, and to read one data bit, HiFi performs three reads and one write. We do not introduce any extra hardware to the memory, and to read one data bit we essentially perform only one read (more precisely, we perform $n+3$ reads to obtain $n-\lceil \log_2n \rceil-1$ data bits). 

If a shift error is detected, HiFi requires two extra bits to be read, thus adding a total of six reads and two writes to the memory. On the other hand, our proposed code does not require any extra read/write operations when it faces a shift error.

If we take the number of read/write operations\footnote{Write operations consume more energy, but we treat read and write operations the same way here. We note that this helps HiFi~\cite{HiFi} as it needs one write per read whereas we do not need such an operation.} needed to read $k$ data bits as a proxy for energy consumption, then we can compare our proposed coding scheme to HiFi~\cite{HiFi} as depicted in Fig.~\ref{Fig:Energy}. We note that this figure only compares the energy consumption of the two methods (in terms of the number of read/write operations), and does not take into account the added complexity and the cost of having extra hardware as needed by~\cite{HiFi}. 

The impact of our scheme on system performance is strictly a function of how it impacts read and write latencies, and this relationship is fixed.  That is, our scheme adds some constant amount of delay to every read and write, and this delay is a linear function of the difference between the length of an extended codeword and the length of a dataword as discussed above. The impact of this fixed memory latency penalty is a function of the use of racetrack (\emph{e.g.}, is it for main memory or non-volatile checkpoint storage or secondary storage) and the frequency with which it is accessed.  An architect studying the use of racetrack memory with our shift error protection scheme would simply modify her simulator by incrementing the latency to read/write the racetrack memory.

==> Hamming.tex <==
Conventional codes are designed for a different error model, bit flips, and are not matched to the challenge of detecting and correcting shift errors. To illustrate why conventional codes are not suitable for racetrack memory, we provide two examples of such codes, namely a single-parity code and an $\left[ 8, 4 \right]$ Hamming code.

% Detecting a shift error is a challenging task that we cover in Section~\ref{Section:Detection}.

\begin{figure}[ht]
\centering
\includegraphics[height = 4cm]{FiguresPDF/SingleParity.pdf}
\caption{A single-parity code cannot detect a shift error nor can it correct one.\label{Fig:SingleParity}}
\end{figure}

\vspace{1mm}
\noindent {\bf Single-parity code:} We start with a single-parity code where the modulo sum of every three bits is stored in the next bit as in Fig.~\ref{Fig:SingleParity}. If any bit, for instance the parity bit, is skipped, then two cases can happen:
\begin{enumerate}

\item $b_5 = 1$: In this case the deletion error is \emph{not} detected, and this undetected error might cause further errors in the subsequent bits. In fact, the deletion might change the entire upcoming sequence of bits resulting in multiple errors. 

\item $b_5 = 0$: In this case, since the parity bit does not match the data, an error is detected. However, the same four bits ($1000$) could result from repetition of $b_3$, or deletion of $b_4$, and the code cannot distinguish between these possibilities.

\end{enumerate} 

\noindent {\bf Hamming code:} Consider an $\left[ 8, 4 \right]$ Hamming code with generator matrix $\mathbf{G}$ given below. 
\begin{align}
G \overset{\triangle}=
\begin{bmatrix}
    1 &0 &0 &0 &0 &1 &1 &1 \\
    0 &1 &0 &0 &1 &0 &1 &1 \\
		0 &0 &1 &0 &1 &1 &0 &1 \\
		0 &0 &0 &1 &1 &1 &1 &0 
\end{bmatrix}
\end{align}
Suppose we want to write dataword $\mathbf{d} = \left[ 0 1 0 1 \right]$, which gets encoded as codeword $\mathbf{c}$:
\begin{align}
\mathbf{c} & = \left[~0~1~0~1~\right]~\mathbf{G} \nonumber \\
& = \left[~0~1~0~1~0~1~0~1~\right].
\end{align}

\begin{figure}[ht]
\centering
\includegraphics[height = 3cm]{FiguresPDF/HammingError.pdf}
\caption{Hamming codes are not suitable error-correcting codes for deletions and repetitions.\label{Fig:HammingError}}
\end{figure}

Consider the situation in Fig.~\ref{Fig:HammingError} in which the stored bit after codeword $\mathbf{c}$ is $0$. If the first bit in $\mathbf{c}$ is deleted, we observe the following binary string:
\begin{align}
\mathbf{c}^\prime = \left[~1~0~1~0~1~0~1~0~\right],
\end{align}
In this case, 
\begin{align}
\mathbf{c}^\prime =  \left[~1~0~1~0~\right]~\mathbf{G},
\end{align}
and the dataword is decoded as $\mathbf{d}^\prime = \left[~1~0~1~0~\right]$. The Hamming code does not detect the error even though all $4$ bits of $\mathbf{d}^\prime$ differ from the corresponding bits in $\mathbf{d}$. We conclude that Hamming codes are not suitable error detecting or correcting codes for shift errors. 

% Therefore, a deletion error causes the Hamming code to decode $\mathbf{d}$ as $\mathbf{d}^\prime$ which corresponds to four errors in four data bits without detecting any errors at all. We conclude that Hamming codes are not suitable error correction codes for shift errors. 

==> Linear.tex <==
For Racetrack memory, one may wonder how well linear codes can perform. In fact from~\cite{}, we know that any linear code that can correct a deletion or a repetition has a storage rate less than or equal to $1/2$. We show that a very simple code can achieve arbitrary close to what is theoretically possible from linear codes.

\noindent {\bf Encoding}: The encoding is simply performed by writing each bit twice in the memory. Suppose $m=1k+3$, if the input data bits are denoted by $d_1,d_2,\ldots,d_k$, then we write the following $m$ bits on the memory:
\begin{align}
\underbrace{d_1 d_1 d_2 d_2 \ldots d_k d_k}_{\text{repetition~code}}\underbrace{100}_{\text{delimiter}}.
\end{align} 

\noindent {\bf Decoding}: Suppose using the delimiter bits we identify a deletion. Then, we must observe an odd number of $0$'s (or $1$'s) in the first $m-4$ bits. Add a single $0$ (or $1$) to this odd number of $0$'s (or $1$'s). Now, bits $b_1, b_3, b_5, \ldots, b_{m-4}$ are the stored data bits.

\noindent {\bf Performance}: The storage rate for this linear code, defined as the number of data bits stored in $m$ bits of the memory, is given by
\begin{align}
R_{\text{repetition}}\left( m \right) \overset{\triangle}= \frac{k}{\underbrace{2k+3}_{=~m}} \overset{m \rightarrow \infty}\rightarrow \frac{1}{2}.
\end{align}

In other words, using linear codes we have at least 100$\%$ overhead, \emph{i.e.} $k$ data bits are mapped to a minimum of $2k$ bits on the memory.

==> Prior.tex <==
There is a limited body of work for error correction in racetrack memory. HiFi~\cite{HiFi} addresses bit deletions in racetrack memory by adding pattern bits at both edges of each track as well as additional read and write ports. The main idea is to read the pattern in parallel with the data bits. If the pattern does not match what was expected, bits are shifted in the reverse direction and the memory is re-read to recover the bits correctly. In order to implement a code that can correct a single deletion, two additional ports (one read and one read/write port) need to be placed in each of the tracks. HiFi assumes a 2D structure for racetrack which allows the addition of extra ports. However, as we discussed in Section~\ref{Section:Racetrack}, racetrack memory achieves high levels of density through its 3D U-shaped geometry which is the preferred structure. In this 3D geometry, adding extra ports will be extremely challenging, if not impossible. As bits are shifted during consecutive reads, some of the pattern bits are ``shifted out'' of the track and virtually get deleted. Thus, for every shift in racetrack, one data bit and two pattern bits are read, while at the same time a new pattern bit is written. The main drawback of this implementation is that it adds substantial physical area and energy overheads because of the additional read and write ports and operations. We also need to emphasize that the placement of additional read and write ports are only feasible because prior work assumes a flat 2D structure for racetrack instead of a U-shaped 3D geometry.

Varshamov-Tenengolts codes have been used for deletion and insertion channels with segmented errors~\cite{liu2010codes} in which deletions {\it or} insertions (but not a mixture of two) could occur. This is a more restrictive model than racetrack memory in which deletions and insertions could both happen. Moreover, if we input $n$ bits to deletion and insertion channels with segmented errors, the output would be a sequence of length $n^\prime$ from which we can easily deduct the number of shift errors. Again, this differs from racetrack memory in which the memory controller is always going to provide the desired number of bits, $n$, regardless of whether an error occurs. Finally, codewords are found using exhaustive search for a given length and the (randomized) construction algorithm adds more overhead compared to our scheme. It is worth noting that the encoding and decoding of~\cite{liu2010codes} are not designed for implementation and introduce extra hardware and energy overheads.

% However, this idea requires the pattern bits to have at least the same length as the data bits as you need to read at least one extra bit for every data bit. Additionally, 


% There is a limited body of work for error correction in racetrack memory. An example is~\cite{HiFi} where the key is adding new hardware. More precisely, in order to detect and correct a shift error of size $i$, $i+1$ additional read/write ports are added. When dealing with single shift errors, every read requires two extra reads and two extra writes to the parity bits. Moreover, the correction is not carried out through coding, rather when an error is detected, a current in the reverse direction is injected to re-read the stored bits. Hence, this method introduces overhead to area, latency, and energy consumption of a racetrack memory design. However, increasing power consumption and latency through adding extra hardware and read/write operations limits the attractiveness of racetrack technology.

==> Problem_Old.tex <==
Racetrack memory consists of a number of read/write ports that are fixed in position and a number of ``tracks'' that store data. To pack more storage per unit surface area, the tracks are packed in a ``U-shape'' format as depicted in Fig.~\ref{}. For simplicity, we choose a 2-D representation as depicted in Fig.~\ref{}. This representation is only used to depict our coding strategy in the following sections. Racetrack memory promises many advantages over the existing technologies such as higher density and much faster access speed. However, in practice the access speed is much slower (up to a $1000\times$) than expected. This is due to the unique error model in Racetrack memory that cannot be simply addressed by ECCs. In what follows, we describe the error model for Racetrack memory.

We assume that each track can store a total of $n$ bits and we assume a total of $s$ tracks. To access a particular position $i_1$ in track $j$ from a current position $i_0$, a specific amount of current, ${\sf I}\left( i_0 \rightarrow i_1 \right)$, is injected in track $\ell$ where the magnitude and sign are determined by $i_0$ and $i_1$ as shown in Fig.~\ref{} (the farther you wish to travel in the track, the higher the magnitude). We refer to $\left| i_1 - i_0 \right|$ as the step size. Let function ${\sf P}\left( \ell \right)$ denote the true position of track $\ell$, and $\hat{{\sf P}}\left( \ell \right)$ denote the system's estimation of the position of track $\ell$, $\ell = 1,2,\ldots,s$. Ideally, we wish 
\begin{align}
{\sf P}\left( \ell \right) = \hat{{\sf P}}\left( \ell \right).
\end{align}
However, this is not always the case as depicted in Fig.~\ref{}. Due to manufacturing imperfections when ${\sf I}\left( i_0 \rightarrow i_1 \right)$ is applied to track $\ell$, we might have
\begin{align}
{\sf P}\left( \ell \right) = i_1 \neq \hat{{\sf P}}\left( \ell \right) = i_1^\prime.
\end{align}
If 
\begin{align}
{\sf P}\left( \ell \right) < \hat{{\sf P}}\left( \ell \right),
\end{align}
then a {\it repetition error} of length $\hat{{\sf P}}\left( \ell \right) - {\sf P}\left( \ell \right)$ has occurred; and if 
\begin{align}
{\sf P}\left( \ell \right) > \hat{{\sf P}}\left( \ell \right),
\end{align}
then a {\it deletion error} of length ${\sf P}\left( \ell \right) - \hat{{\sf P}}\left( \ell \right)$ has occurred. In general as $\left| i_1 - i_0 \right|$ increases, so does the probability of having a deletion or an insertion error. 

Our goal is to devise a coding strategy that would allow reliable data recovery in presence of deletion and repetition errors in Racetrack memory.

==> Related.tex <==
Varshamov-Tenegolts codes have been used for deletion and insertion channels with segmented errors~\cite{liu2010codes} in which a number of deletions or insertions (but not a mixture of two) could occur. This is a more restrictive model than racetrack memory in which deletions and insertions could both happen. Moreover, if we input $n$ bits to deletion and insertion channels with segmented errors, the output would be a sequence of length $n^\prime$ from which we can easily deduct the number of shift errors. Again, this differs from racetrack memory in which the memory controller is always going to provide the desired number of bits, $n$, regardless of whether an error occurs.

Finally, codewords are found using exhaustive search for a given length and the (randomized) construction algorithm adds more overhead compared to our scheme. It is worth noting that the encoding and decoding of~\cite{liu2010codes} are not designed for implementation and introduce extra hardware and energy overheads.

==> SingleDeletion.tex <==
We focus on a single track. We detect and correct a single deletion error every $m-1$ shifts or equivalently every $m$ bits. We first describe the encoding and decoding and then clarify the ideas through an example. We do detection and correction separately. The key is the correction and detection is done through a simple trick that we refer to as ``delimiter bits.'' 

\noindent {\bf Detection:} To detect a single deletion, we use the following format. We use bits $1,2,\ldots,m-2$ to store data and we set bits $m-1$ and $m$ to $1$ and $0$ respectively; bits $m+1,m+2,\ldots,2m-2$ to store data and we set bits $2m-1$ and $2m$ to $1$ and $0$ respectively and so on. Consider the first $m$ bits as depicted in Fig.~\ref{}. We refer to the ``$10$'' pattern in positions $m-1$ and $m$ as the delimiter bits. Now, if any of the first $m-1$ bits ($b_1,b_2,\ldots,b_{m-2}$ and $p_1$) gets deleted then once we read the data, in position $m-1$ we obtain a $0$. This indicates a single deletion in the first $m-1$ bits. On the other hand, if bit $m$ gets deleted, the first $m-1$ bits have been retrieved correctly and we delay the detection to the next $m$ bits.

\noindent {\bf Correction:} Consider two sequences of bits $\vec{b} = b_1,b_2,\ldots,b_{n}$ and $\vec{c} = c_1,c_2,\ldots,c_{n}$. In order to be able to use these two sequences to store different values in the memory, we need to be able to distinguish them even after a single deletion. In other words, if $b_i$ and $c_j$ are deleted $i,j \in \{ 1,2,\ldots, n \}$, then the resulting sequences should not be identical. If two bit sequences $\vec{b}$ and $\vec{c}$ can be confused with a single deletion, we refer to them as conflicting and denote it by $\vec{b} \sim \vec{c}$; and if cannot be confused with a single deletion, we refer to them as non-conflicting and denote it by $\vec{b} \nsim \vec{c}$. Therefore, our goal is to find the maximum number of sequences of length $n$ such that each pair is non-conflicting. This problem can be nicely defined and solved in graph theoretical terms.

Consider all $2^{n}$ sequences of length $n$. We create a conflict graph $N = \left( \mathcal{V}, \mathcal{E} \right)$, where $\mathcal{V}$ is the node set and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the edge set. Each node in this graph corresponds to a unique binary sequence of length $m-2$ ($\left| \mathcal{V} \right| = 2^n$). For simplicity label the nodes with numbers $0,1,2,\ldots,2^{n}-1$ and let node $i$ correspond to the binary expansion $i$. Now, $\left( i, j \right) \in \mathcal{E}$ if and only if the binary expansions of $i$ and $j$ are conflicting. In this graph, a set of non-conflicting sequences corresponds to an {\it independent set}; and the maximum number of sequences of length $n$ corresponds to the size of the {\it maximum independent set}. This problem is well studied and understood in graph theory and we can calculate the size of the maximum independent set for various values of $n$, $\left| \mathcal{I}^n_{\sf max} \right|$. We use the binary sequences corresponding to the nodes in the maximum independent set as our codewords.

A useful bound~\cite{} gives us
\begin{align}
\left| \mathcal{I}^n_{\sf max} \right| \geq \frac{2^n}{n+1}.
\end{align}
Thus, considering the delimiter bits, we guarantee a storage rate, $R_n$, such that
\begin{align}
\label{Eq:RateLowerBound}
R_n \geq \frac{n-\log_2\left( n+1 \right) - 2}{n}.
\end{align}
For instance, we have $R_{32} \geq 0.75$. We note that (\ref{Eq:RateLowerBound}) gives us a lower-bound and for finite values of $n$, the rate is in fact better than the lower-bound. Moreover, we note that $\lim_{n \rightarrow \infty} R_n = 1$.

\noindent {\bf Encoding:} For a fixed $n$, we have $\left| \mathcal{I}^n_{\sf max} \right|$ non-conflicting sequences and thus, we can store $\log_2\left| \mathcal{I}^n_{\sf max} \right|$ data bits using such sequences. Sort the nodes $v_i \in \mathcal{I}^n_{\sf max}$ according to their indices so that
\begin{align}
\mathcal{I}^n_{\sf max} = \left\{ \hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{\mathcal{I}^n_{\sf max}} \right\}.
\end{align}
Now, a data sequence corresponding to a value $D$ between $0$ and $2^{\left| \mathcal{I}^n_{\sf max} \right|}$ is mapped to $\hat{v}_{\text{binary~exp.~of~}D}$. 


\noindent {\bf Decoding:} Using our delimiter sequence, we can detect a single deletion. If no deletion happens, and we obtain $\hat{v}_j$ then the stored data is simply $j$. However, if a single deletion happens, we need to identify which $\hat{v}_j$ was initially stored. Let $\mathcal{D}_{\hat{v}_j}$ denote the set of all sequences of length $n-1$ that result from a single deletion from $\hat{v}_j$. Based on our construction, we have
\begin{align}
\mathcal{D}_{\hat{v}_i} \cap \mathcal{D}_{\hat{v}_j} = \emptyset, \qquad \forall~i \neq j,~\hat{v}_i,\hat{v}_j \in \mathcal{I}^n_{\sf max}.
\end{align}
Thus, given a sequence of length $n-1$ resulting from a single deletion from $\hat{v}_j$, uniquely identifies $\hat{v}_j$. Once we have $\hat{v}_j$, we know the stored value. Note that in general, we do {\it not} have  $\left| \mathcal{D}_{\hat{v}_i} \right| = \left| \mathcal{D}_{\hat{v}_j} \right|$.

\noindent {\bf A Single-Deletion Code of length $n = 5$:} After deriving the maximum independent set for $n=5$, we have the following six codewords to use: 
\begin{align}
\hat{v}_1 &\rightarrow 00000, \nonumber \\
\hat{v}_2 &\rightarrow 00011, \nonumber \\
\hat{v}_3 &\rightarrow 01110, \nonumber \\
\hat{v}_4 &\rightarrow 10101, \nonumber \\
\hat{v}_5 &\rightarrow 11000, \nonumber \\
\hat{v}_6 &\rightarrow 11111. \nonumber 
\end{align} 
We note that there might be more than one maximum independent sets for each value of $n$. Note that a single deletion does not create any confusion between these cosewords. Moreover, note that $\mathcal{D}_{\hat{v}_1} = \left\{ 0000 \right\}$ and $\mathcal{D}_{\hat{v}_4} = \left\{ 0101, 1101,1001,1011,1010 \right\}$. Now, if we read out ``$0101$'' we know that we used codeword $\hat{v}_4 \rightarrow 10101$ and the stored data is $4$. Finally as mentioned before, we need to use the delimiter bits to store our data. So, if we want to store $2,4,$ and $5$ then on the memory we write:
$$\underbrace{00011}_{\hat{v}_2}\mathbf{10}\underbrace{10101}_{\hat{v}_4}\mathbf{10}\underbrace{11000}_{\hat{v}_5}\mathbf{10}.$$


==> SingleDeletionConcept.tex <==
Our goal in this subsection is to show how one can use a graph-based code to correct a single deletion error. We first describe the key idea and present an example. We then formally define this code. We note that the idea of using graph-based codes to correct deletion errors has been previously used for communication systems~\cite{Sloane}. We assume that error detection is already performed using the delimiter bits introduced in the previous section. We denote binary strings with boldface letters, \emph{e.g.}, $\mathbf{x}$, and bits in these strings are denoted by lowercase letters, \emph{e.g.}, $x_1$. To label different binary strings, we use different boldface letters, \emph{e.g.}, $\mathbf{x}$ and $\mathbf{y}$. % , or we may use subscripts for the boldface letters, \emph{e.g.}, $\mathbf{x}_1$ and $\mathbf{x}_2$.

\noindent {\bf Key idea:} Consider two binary strings $\mathbf{x} = x_1,x_2,\ldots,x_{n}$ and $\mathbf{y} = y_1,y_2,\ldots,y_{n}$. In order to be able to use these two strings to store different values in racetrack memory, we need to be able to distinguish them even after a single deletion. In other words, if $x_i$ and $y_j$ are deleted for $i,j \in \{ 1,2,\ldots, n \}$, then the resulting binary strings should not be identical. If two binary strings $\mathbf{x}$ and $\mathbf{y}$ can be confused with a single deletion, we refer to them as {\it conflicting} with regards to deletion; if they cannot be confused with a single deletion, we refer to them as {\it non-conflicting} with regards to deletion. Consider the following set of binary strings.
\begin{align}
\label{Eq:CodewordsExample}
\left\{ \underbrace{00000}_{\mathbf{c}_0}, \underbrace{00011}_{\mathbf{c}_1}, \underbrace{01110}_{\mathbf{c}_2}, \underbrace{10101}_{\mathbf{c}_3}, \underbrace{11000}_{\mathbf{c}_4}, \underbrace{11111}_{\mathbf{c}_5} \right\}.
\end{align}

These six strings/codewords are pairwise non-conflicting. Let $D_{\mathbf{c}_j}$ denote the set of all strings of length $4$ that result from a single deletion in $\mathbf{c}_j$. In this example, $D_{\mathbf{c}_0} = \left\{ 0000 \right\}$ and $D_{\mathbf{c}_3} = \left\{ 0101, 1101,1001,1011,1010 \right\}$. Thus, if we read out ``$0101$'' we know that it refers to codeword $\mathbf{c}_3 = 10101$. 

Using the codewords of (\ref{Eq:CodewordsExample}), we can store six different values, say $0,1,\ldots,5$. So, if we want to store values $2,4,$ and $5$ to memory, the actual bits written to memory are:
\begin{align}
\label{Eq:CodeOnMemory}
\underbrace{01110}_{\mathbf{c}_2}\underbrace{\mathbf{100}}_{\text{delimiter}}\underbrace{11000}_{\mathbf{c}_4}\underbrace{\mathbf{100}}_{\text{delimiter}}\underbrace{11111}_{\mathbf{c}_5}\underbrace{\mathbf{100}}_{\text{delimiter}}.
\end{align}

\noindent {\bf Formal definition:} Consider all $2^{n}$ binary strings of length $n$. We create a conflict graph $N = \left( V, E \right)$, where $V$ is the node set and $E \subseteq V \times V$ is the edge set. Each node in this graph corresponds to a unique binary string of length $n$ ($\left| V \right| = 2^n$). For simplicity, label the nodes with numbers $0,1,2,\ldots,2^{n}-1$ and let node $i$ correspond to the binary expansion (of length $n$) of $i$ that we denote by $\mathbf{b}_i$. 

Now, $\left( i, j \right) \in E$ if and only if $\mathbf{b}_i$ and $\mathbf{b}_j$ are conflicting. In this graph, a set of non-conflicting strings corresponds to an {\it independent set}; the maximum number of strings of length $n$ corresponds to the size of the {\it maximum independent set}. For a given $n$, denote the maximum independent set by $I_n$. We use the binary strings corresponding to the nodes in the maximum independent set as our codewords. We note that the maximum independent set of a graph is not necessarily unique.

\noindent {\bf Encoding and decoding:} For a fixed $n$, we have $\left| I_n \right|$ non-conflicting strings and thus, we can store $\log_2\left| I_n \right|$ (for now assume this number is an integer) data bits using such strings. If $\mathbf{c}_i, \mathbf{c}_j \in I_n$ then $D_{\mathbf{c}_i} \neq D_{\mathbf{c}_j}$, thus decoding can be perofrmed by identifying from which codeword the observed sequence is obtained from.

The downside of encoding and decoding as described above is that you need to use a lookup table to find the right codeword. Using a lookup table is practical for short codewords but as the codeword length increases, the lookup table grows exponentially in size.

\begin{table*}[t!]
\begin{center}
\begin{tabular}{|K{\columnwidth}|K{\columnwidth}|N}
\hline
{\bf Encoding Algorithm}                                 & {\bf Example for $n=8,~\ell = 3$} &\\[10pt] \hline
{\bf Step~1}: Start with a zero-vector $\mathbf{c}$ of length $n = 2^\ell$.    &  $\mathbf{c} = c_1c_2\ldots c_8 = 00000000$ &\\[10pt] \hline
{\bf Step~2}: Set positions that are not powers of two to data bits.  & $\mathbf{d} = 1011~\rightarrow~\mathbf{c} = 00\underline{1}0\underline{011}0$ &\\[9pt] \hline
{\bf Step~3}: Calculate the checksum $\sum_{i=1}^n{ic_i}$.   & $\sum_{i=1}^n{ic_i} = 3 + 6 + 7 = 16$  &\\[9pt] \hline
{\bf Step~4}: Set $s$ to be the minimum value that needs to be added to the checksum to make it equal to $0$ modulo $n+1$.       &  $s=2$   &\\[20pt] \hline
{\bf Step~5}: Set the $\ell+1$ positions that are powers of two to the binary expansion (of length $\ell+1$) of $s$. Start from $c_1$ and set it to the least significant bit (LSB) of the binary expansion of $s$, and move all the way to $c_n$ and set it to the most significant bit (MSB) of the binary expansion of $s$.  & $s = \left( 0010 \right)_2~\rightarrow~c_1 = 0,~c_2 = 1,~c_4 = 0,~c_8 = 0 \newline \rightarrow~\mathbf{c} = \underline{01}1\underline{0}011\underline{0}$   &\\[30pt]\hline 
\end{tabular}
\vspace{2mm}
\caption{Encoding algorithm alongside an example for $n=8$.\label{Table:Encoding}}
\end{center}
\end{table*}

\begin{table*}[ht!]
% \large
\begin{center}
\begin{tabular}{|K{\columnwidth}|K{\columnwidth}|N}
\hline
{\bf Deletion Correction Algorithm}                                 & {\bf Example for $n=8,~\ell = 3$} &\\[10pt] \hline
{\bf Step~1}: Suppose a codeword $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ from $VT\left( n \right)$ is stored in racetrack memory, and using the delimiter bits, we identify a single deletion, and we observe $\mathbf{c}^\prime =  \left( c^\prime_1, c^\prime_2, \ldots, c^\prime_{n-1} \right)$.    &  $\mathbf{c} = 011001\underline{1}0~\rightarrow~\mathbf{c}^\prime = 0110010$ &\\[30pt] \hline
{\bf Step~2}: Set $\omega$ to be the Hamming weight (number of $1$'s) of $\mathbf{c}^\prime$.  & $\omega=3$ &\\[12pt] \hline
{\bf Step~3}: Calculate the checksum $\sum_{i=1}^{n-1}ic^\prime_i$. & $\sum_{i=1}^{7}ic^\prime_i = 11$ &\\[9pt] \hline
{\bf Step~4}: Set $s$ to be the minimum amount that needs to be added to the checksum in order to make it $0~\textbf{mod}~n+1$.  & $s = 7$ &\\[20pt] \hline
{\bf Step~5}: If $s \leq \omega$, we restore the codeword by adding a $0$ immediately to the left of the rightmost $s$ $1$'s. Otherwise, we restore the codeword by adding a $1$ immediately to the right of the leftmost $\left( s-\omega-1 \right)$ $0$'s.   & $e>\omega~\rightarrow~$restore the codeword by adding a $1$ immediately to the right of the leftmost $\left( s-\omega-1 \right) = 3$ zeros to arrive at the correct codeword: $01100\underline{1}10$.               &\\[30pt] \hline
\end{tabular}
\vspace{2mm}
\caption{Deletion Correction Algorithm alongside an example for $n=8$.\label{Table:Decoding}}
\end{center}
\end{table*}


We have the following result for the graph-based codes introduced in this section which proves that these codes can be used to correct a single insertion (and therefore, a single repetition) as well as a single deletion.
\begin{lemma}
\label{Lemma:DeletionandInsertion}
If two binary strings are non-conflicting with regards to deletion, then they are non-conflicting with regards to insertion.
\end{lemma}
\begin{proof}
Suppose two binary strings $\mathbf{x}$ and $\mathbf{y}$ of length $n$ are non-conflicting with regards to deletion but conflicting with respect to insertion. Suppose inserting $x^\prime$ in position $i$ of $\mathbf{x}$ and $y^\prime$ in position $j$ of $\mathbf{y}$ results in the same sequence of length $n+1$. Without loss of generality, we assume $i \leq j$. This implies that deleting $x_{j-1}$ and $y_{i}$ from $\mathbf{x}$ and $\mathbf{y}$ respectively, would result in the same sequence of length $n-1$. This contradicts the assumption that $\mathbf{x}$ and $\mathbf{y}$ are non-conflicting with regards to deletion, thus proving the lemma.
\end{proof}

It is also worth noting an important difference between the graph based codes and conventional error-correcting codes. In conventional ECCs, Hamming distance defines a sphere around each codeword and if this sphere has radius $t$, then their centers are codewords of a $\left(2t + 1\right)$-error-correcting code. Graph-based codes do not rely on Hamming distance but they rather rely on having disjoint sub-strings of length $n-1$ as denoted by $D_{{\mathbf{c}}_j}$ above. Unlike conventional ECCs where all spheres have equal radius, these disjoint sets associated with the graph-based codewords do not all have the same size as we saw for the codewords in (\ref{Eq:CodewordsExample}).

==> Submission ISIT 2017/AlgoDescription.tex <==
In this appendix, we prove Lemma~\ref{Lemma:VTGraphBased}. To prove the result, it suffices to show that after a single deletion, Varshamov-Tenengolts codes cannot be confused and unique recovery is guaranteed. We borrow from the argument given in~\cite{Sloane}. 

Suppose a codeword $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ from $VT\left( n \right)$ is stored in Racetrack memory; and bit $x \in \{ 0, 1 \}$ in position $1 \leq p \leq n$ is deleted to observe $\mathbf{c}^\prime = \left( c^\prime_1, c^\prime_2, \ldots, c^\prime_{n-1} \right)$. Let there be $L_0$ $0$'s and $L_1$ $1$'s to the left of $x$, and $R_0$ $0$'s and $R_1$ $1$'s to the right of $x$ (with $p = 1 + L_0 + L_1$). Also, let $\omega$ denote the weight (number of $1$'s) of $\mathbf{c}^\prime$. Calculate the new checksum $\sum_{i=1}^{n-1}ic^\prime_i$.

Now if $x = 0$, the new checksum is $R_1$ less than $\sum_{i=1}^{n}ic_i$. We note that $R_1 \leq \omega$. If $x = 1$, the new checksum is $p+R_1$ less than $\sum_{i=1}^{n}ic_i$. We note that $p+R_1 = 1 + L_0 + L_1 + R_1 = 1 + \omega + L_0$ which is greater than $\omega$.

So if the deficiency in the checksum is less than or equal to $\omega$, we restore the codeword by adding a $0$ just to the left of the rightmost $R_1$ $1$'s. Otherwise, we restore the codeword by adding a $1$ just to the right of the leftmost $L_0$ $0$'s.



==> Submission ISIT 2017/Beyond.tex <==
In Section~\ref{Section:Racetrack}, we assumed that in every $m-1$ shifts at most one shift error may occur. In this section, we take the first steps in relaxing this assumption and we discuss the challenges that arise by doing so. In particular, we assume the memory behaves {\it mostly} in accordance with the assumption stated above. However, occasionally a combination of one deletion and one repetition may occur within $m-1$ shifts. Moreover, if we have one deletion and one repetition in $m-1$ consecutive shifts, then we do not see another shift error for at least $2(m-1)$ following shifts. This latter assumption is to guarantee proper error detection. 

We first need to describe how to detect a combination of one deletion and one repetition. We then use an outer-code on top of the code presented in Section~\ref{Section:Practical} to correct such errors. We have the following result for VT codes.
\begin{lemma}
\label{Lemma:combination}
For any two binary strings  $\mathbf{x}, \mathbf{y} \in VT\left( n \right)$, $\mathbf{y}$ cannot be obtained from $\mathbf{x}$ by a deletion followed by an insertion (or by an insertion followed by a deletion).
\end{lemma}

\begin{proof}
Suppose $\mathbf{x}^\prime \in D_{-1}\left( \mathbf{x} \right)$ and $\mathbf{y}^\prime \in D_{-1}\left( \mathbf{y} \right)$. If $\mathbf{y}$ can be obtained from $\mathbf{x}$ by a deletion followed by an insertion, then 
\begin{align}
D_{+1}\left( \mathbf{x}^\prime \right) \cap D_{+1}\left( \mathbf{y}^\prime \right) \neq \emptyset.
\end{align}
In other words, $\mathbf{x}$ and $\mathbf{y}$ do not satisfy (\ref{Eq:CodeRequirement}). However, this contradicts Lemma~\ref{Lemma:VTGraphBased}. This contradiction proves the result. A similar argument can be used when an insertion is followed by a deletion. 
\end{proof}

Lemma~\ref{Lemma:combination} immediately results in the following observation.
\begin{corollary}
A combination of a deletion error and an insertion error on $\mathbf{x} \in VT\left( n \right)$ either results in $\mathbf{x}$ or in $\mathbf{y} \notin VT\left( n \right)$ (an invalid codeword).
\end{corollary}

To detect a combination of one deletion error and one insertion (or repetition) error, we can no longer solely rely on the delimiter bits. First assume no shift error happens within the delimiter bits. To detect a combination of errors, we need to calculate the check-sum as we read the stored bits. If the stored codeword between two sets of delimiter bits  $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ does not pass the check-sum constraint of (\ref{eq:VTCondition}), and the delimiter bits do not reveal any errors, we conclude that a combination of one deletion error and one insertion error has happened. 

Now suppose we detect a combination of one deletion error and one insertion (or repetition) error by observing an invalid codeword as described above. We can use an outer-code to recover data in this case as illustrated in Fig.~\ref{Fig:OuterCode} where the outer-code is a simple single parity code. We note that we use VT codes to correct single shift errors and to detect a combination deletion and repetition errors.

Next, we need to understand what happens if one (or two) error happens within the delimiter bits. To see why this issue requires attention, consider the delimiter bits $(100)$ and suppose the first bit is deleted and the second bit is repeated. Thus, when we read the memory we observe $000$ instead of the $100$ pattern. According to Table~\ref{Table:Syndrom}, this observation corresponds to a deletion in the first $m-3$ shifts which is not correct.
Since we assumed that no more shift errors happen for at least $2(m-1)$ shifts after a combination of deletion and repetition errors, we can identify this false detection using the next set of delimiter bits. In particular, when we observe the following $100$ pattern, we update our previous error detection accordingly. Thus, we need to wait to see the next set of delimiter bits before we attempt to recover data from the memory.

In this section, we only considered having a combination of one deletion and one repetition. Dealing with other combinations of two shift errors (\emph{e.g.}, two deletions) is more challenging. First is the issue of detection. The delimiter bits we introduced in this paper work well for detecting a single shift error and we could use them with the VT codes to detect a combination of one deletion and one repetition. However, it is not an easy task to modify them in order to detect two deletion errors or two repetition errors. Error detection for multiple shift errors is an interesting subject for future work. 

Second is the issue of correction. Conceptually we can design codes that can correct multiple shift errors. However, the encoding complexity quickly increases. Unfortunately, we are not aware of codes that similar to VT codes have reasonable encoding and decoding complexity. However, we believe exploiting the spatial diversity of racetrack technology (having multiple tracks in parallel) may enable us to correct multiple shift errors once they are detected.

==> Submission ISIT 2017/Conclusion.tex <==
We introduced a single-shift-error-detecting (SSED) single-shift-error-correcting (SSEC) code for racetrack memory. Our code does not require any hardware modifications and has a storage overhead that is logarithmic in the length of the codeword. We separated detection from correction to make the common case in which no error happens, fast and efficient. We showed how non-linear graph-based codes are suitable for error correction in racetrack technology. We then focused on a specific subclass of such codes, namely Varshamov-Tenengolts codes, for which we introduced an encoding algorithm. Our proposed code is amenable to to fast encoding and decoding algorithms. We investigated the storage cost (rate) and the performance of our code, and quantified its performance and demonstrated its gain over linear codes.

The next steps include detection and correction of bit flip errors on top of shift errors. Moreover, we aim to design codes that can detect and correct multiple shift errors.

==> Submission ISIT 2017/Delimiter.tex <==
In Section~\ref{Section:Detection}, we introduced delimiter bits to separate error detection from error correction, and we chose $100$ as delimiter bits. Here, we reveal the rationale for this choice. 

A brute force search shows that we cannot detect a shift error and its type (deletion vs. repetition) using fewer than three bits. Say we use three bits $a,b,$ and $c$ as delimiter bits. The top priority is to detect a shift error and its type in the first $m-3$ shifts since that would directly affect the bits stored prior to delimiter bits. We summarize the resulting observations in positions $m-2$, $m-1$ and $m$ for a shift error in the first $m-3$ shifts in Table~\ref{Table:SyndromRationale}.

\begin{table}[ht]
\begin{center}
\begin{tabular}{L|M|M|M|N}
\cline{2-4}
																				                       & position $m-2$ & position $m-1$ & position $m$ &\\[10pt] \hline
\multicolumn{1}{|L|}{no error}                                 & $a$              & $b$              & $c$      &\\[10pt] \hline
\multicolumn{1}{|L|}{$1$ deletion in the first $m-3$ shifts}   & $b$              & $c$              & {\sf X}  &\\[10pt] \hline
\multicolumn{1}{|L|}{$1$ repetition in the first $m-3$ shifts} & {\sf X}          & $a$              & $b$      &\\[10pt] \hline 
\end{tabular}
\vspace{2mm}
\caption{Resulting observations in positions $m-2$, $m-1$ and $m$ for a shift error in the first $m-3$ shifts. Symbol ${\sf X}$ can be either a zero or a one.\label{Table:SyndromRationale}}
\end{center}
\end{table}

To guarantee that a shift error and its type can be detected, it suffices to have $a \neq b$ and $a \neq c$. The reason is that $a \neq b$ makes the error-free observations different from those resulted from a deletion or a repetition. Moreover, $a \neq c$ makes the observations resulted from a deletion different from those resulted from a repetition. We chose $abc = 100$ based on the argument presented here.


==> Submission ISIT 2017/Detection.tex <==
In this section, we introduce delimiter bits to detect a single deletion or a single repetition in every $m-1$ shifts. 

\begin{figure}[ht]
\centering
\includegraphics[width = \columnwidth]{FiguresPDF/Delimiter.pdf}
\caption{Every $m$ bits, we allocate three delimiter bits, $100$, for the purpose of error detection.\label{Fig:Delimiter}}
\end{figure}

Consider $m$ consecutive magnetic domains in racetrack memory. If no error happens, we need $m-1$ shifts to access and read the $m$ bits stored in these $m$ domains. We have the following result for detecting a single shift error every $m-1$ shifts.
\begin{claim}
We can detect a single shift error and its type (deletion vs. repetition) using three out of every $m$ magnetic domains in racetrack memory.
\end{claim}

\begin{proof}
In every $m$ magnetic domains, we set the last three to predetermined bits $1,0,$ and $0$ as shown in Fig.~\ref{Fig:Delimiter}. We refer to the ``$100$'' pattern in positions $m-2$, $m-1$ and $m$ as the ``delimiter bits.'' 


\begin{table}[ht]
\begin{center}
\begin{tabular}{L|M|M|M|}
\cline{2-4}
																				                       & position $m-2$ & position $m-1$ & position $m$ \\ \hline
\multicolumn{1}{|L|}{no error}                                 & 1              &  0             &  0           \\ \hline
\multicolumn{1}{|L|}{$1$ deletion in the first $m-3$ shifts}   & {\bf 0}        & 0              & {\sf X}      \\ \hline
\multicolumn{1}{|L|}{$1$ repetition in the first $m-3$ shifts} & {\sf X}        & {\bf 1}        & 0            \\ \hline \rowcolor{Gray}
\multicolumn{1}{|L|}{$1$ deletion in the last $2$ shifts}      & 1              & 0              & {\sf X}      \\ \hline \rowcolor{Gray}
\multicolumn{1}{|L|}{$1$ repetition in the last $2$ shifts}    & 1              & 0              & 0            \\ \hline
\end{tabular}
\vspace{2mm}
\caption{Resulting observations in positions $m-2$, $m-1$ and $m$ for all possible error combinations. \label{Table:Syndrom}}
% Symbol ${\sf X}$ can be either a zero or a one.
\end{center}
\end{table}

We summarize the resulting observations in positions $m-2$, $m-1$ and $m$ for all possible error combinations in Table~\ref{Table:Syndrom}. A deletion or a repetition in the first $m-3$ shifts (or the first $m-2$ observed bits) can be identified since the resulting observations in positions $m-2$, $m-1$, and $m$ do not match the $100$ pattern. For instance, if we observe a $0$ in position $m-2$, we know a deletion in the first $m-3$ shifts has happened.

The two shaded possibilities are more subtle. Suppose a repetition happens in the final two shifts. Then the resulting observation is $100$ which matches the error-free case. Interestingly, this is not a problem for the following reason. First we note that the data is stored only in the first $m-3$ bits and a repetition in the final two shifts does not affect that data. However, this error affects the stored data that follows. But since we assume at most one shift error every $m-1$ shifts, until the next set of delimiter bits, no other shift errors happen. As a result, the repetition error will be detected by the following delimiter bits. 
\end{proof}

We use the delimiter bits between $n$-bit codewords. We refer to a codeword plus the immediate delimiter bits as an {\it extended codeword} of length $m = n +3$.


==> Submission ISIT 2017/Eval.tex <==
In this section, we investigate the storage cost (rate) and the performance of our code. As mentioned earlier, our code achieves a storage rate of 
\begin{align*}
R_{\text{VT}}\left( m \right) = \frac{m - \log_2(m-3) - 4}{m}.
\end{align*}
We plotted this rate for $m$ from $11$ ($2^3+3$) to $131$ ($2^7+3$) in Fig.~\ref{Fig:Rate}. This rate approaches $1$ as $m$ increases. In this figure, we also plotted the theoretical performance of the best linear code for racetrack memory. Even at moderate values of $m$, our code provides a significant gain over the linear code. For instance at $m = 35$ ($2^5 + 3$), our code has a rate of $0.743$ which corresponds to a $62.5\%$ improvement in terms of storage overhead compared to the linear code's rate ($0.457$). This gain approaches $100\%$ as $m$ increases. 

Besides rate, it is important to pay attention to the energy consumption of our scheme. HiFi~\cite{HiFi} detects and corrects a shift error by adding two extra read/write ports, and to read one data bit, HiFi performs three reads and one write. We do not introduce any extra hardware to the memory, and to read one data bit we essentially perform only one read (more precisely, we perform $n+3$ reads to obtain $n-\lceil \log_2n \rceil-1$ data bits). 

If a shift error is detected, HiFi requires two extra bits to be read, thus adding a total of six reads and two writes to the memory. On the other hand, our proposed code does not require any extra read/write operations when it faces a shift error.

If we take the number of read/write operations\footnote{Write operations consume more energy, but we treat read and write operations the same way here. We note that this helps HiFi~\cite{HiFi} as it needs one write per read whereas we do not need such an operation.} needed to read $k$ data bits as a proxy for energy consumption, then we can compare our proposed coding scheme to HiFi~\cite{HiFi} as depicted in Fig.~\ref{Fig:Energy}. We note that this figure only compares the energy consumption of the two methods (in terms of the number of read/write operations), and does not take into account the added complexity and the cost of having extra hardware as needed by~\cite{HiFi}. 

The impact of our scheme on system performance is strictly a function of how it impacts read and write latencies, and this relationship is fixed.  That is, our scheme adds some constant amount of delay to every read and write, and this delay is a linear function of the difference between the length of an extended codeword and the length of a dataword as discussed above. The impact of this fixed memory latency penalty is a function of the use of racetrack (\emph{e.g.}, is it for main memory or non-volatile checkpoint storage or secondary storage) and the frequency with which it is accessed.  An architect studying the use of racetrack memory with our shift error protection scheme would simply modify her simulator by incrementing the latency to read/write the racetrack memory.

==> Submission ISIT 2017/Hamming.tex <==
Conventional codes are designed for a different error model, bit flips, and are not matched to the challenge of detecting and correcting shift errors. To illustrate why conventional codes are not suitable for racetrack memory, we provide two examples of such codes, namely a single-parity code and an $\left[ 8, 4 \right]$ Hamming code.

% Detecting a shift error is a challenging task that we cover in Section~\ref{Section:Detection}.

\begin{figure}[ht]
\centering
\includegraphics[height = 4cm]{FiguresPDF/SingleParity.pdf}
\caption{A single-parity code cannot detect a shift error nor can it correct one.\label{Fig:SingleParity}}
\end{figure}

\vspace{1mm}
\noindent {\bf Single-parity code:} We start with a single-parity code where the modulo sum of every three bits is stored in the next bit as in Fig.~\ref{Fig:SingleParity}. If any bit, for instance the parity bit, is skipped, then two cases can happen:
\begin{enumerate}

\item $b_5 = 1$: In this case the deletion error is \emph{not} detected, and this undetected error might cause further errors in the subsequent bits. In fact, the deletion might change the entire upcoming sequence of bits resulting in multiple errors. 

\item $b_5 = 0$: In this case, since the parity bit does not match the data, an error is detected. However, the same four bits ($1000$) could result from repetition of $b_3$, or deletion of $b_4$, and the code cannot distinguish between these possibilities.

\end{enumerate} 

\noindent {\bf Hamming code:} Consider an $\left[ 8, 4 \right]$ Hamming code with generator matrix $\mathbf{G}$ given below. 
\begin{align}
G \overset{\triangle}=
\begin{bmatrix}
    1 &0 &0 &0 &0 &1 &1 &1 \\
    0 &1 &0 &0 &1 &0 &1 &1 \\
		0 &0 &1 &0 &1 &1 &0 &1 \\
		0 &0 &0 &1 &1 &1 &1 &0 
\end{bmatrix}
\end{align}
Suppose we want to write dataword $\mathbf{d} = \left[ 0 1 0 1 \right]$, which gets encoded as codeword $\mathbf{c}$:
\begin{align}
\mathbf{c} & = \left[~0~1~0~1~\right]~\mathbf{G} \nonumber \\
& = \left[~0~1~0~1~0~1~0~1~\right].
\end{align}

\begin{figure}[ht]
\centering
\includegraphics[height = 3cm]{FiguresPDF/HammingError.pdf}
\caption{Hamming codes are not suitable error-correcting codes for deletions and repetitions.\label{Fig:HammingError}}
\end{figure}

Consider the situation in Fig.~\ref{Fig:HammingError} in which the stored bit after codeword $\mathbf{c}$ is $0$. If the first bit in $\mathbf{c}$ is deleted, we observe the following binary string:
\begin{align}
\mathbf{c}^\prime = \left[~1~0~1~0~1~0~1~0~\right],
\end{align}
In this case, 
\begin{align}
\mathbf{c}^\prime =  \left[~1~0~1~0~\right]~\mathbf{G},
\end{align}
and the dataword is decoded as $\mathbf{d}^\prime = \left[~1~0~1~0~\right]$. The Hamming code does not detect the error even though all $4$ bits of $\mathbf{d}^\prime$ differ from the corresponding bits in $\mathbf{d}$. We conclude that Hamming codes are not suitable error detecting or correcting codes for shift errors. 

% Therefore, a deletion error causes the Hamming code to decode $\mathbf{d}$ as $\mathbf{d}^\prime$ which corresponds to four errors in four data bits without detecting any errors at all. We conclude that Hamming codes are not suitable error correction codes for shift errors. 

==> Submission ISIT 2017/Introduction.tex <==
Historically, improvements in memory and storage have been due to advances in the memory technologies themselves together with innovations by computer architects who design memory and storage systems, and by coding theorists who design codes for storing data.

Racetrack memory is a non-volatile memory engineered to provide both high density and low latency, and aims to replace conventional memories such as DRAM and Flash. Racetrack memory stores data in ``tape-like'' tracks, and to read a stored bit, an electric current is injected to place the desired bit under the read-write port. Tracks can be manufactured in two or three dimensions, but the U-shaped three-dimensional geometry shown in Fig.~\ref{Fig:Racetrack3D} is preferred because it significantly increases recording density. Prior work on error resilience assumed multiple read/write ports on a single track, but this geometry requires a single read/write port. Competing technologies, such as phase-change memory (PCM) and magneto-resistive random-access memory (MRAM) cannot match the density of racetrack memory. In terms of latency, only SRAM (which is a volatile technology) has a slight advantage, but it comes at the cost of lower density~\cite{mittalsurvey,thomas2011racetrack,sun2013cross}. 

Racetrack uses current injection to {\it shift} magnetic domains that store data bits on the tracks. In this technology, a deletion occurs when the injected current is larger than expected causing one or more domains to be skipped. A repetition occurs when the injected current is smaller than expected, so that the domain under the port does not change, and we read the same bit two or more times. We refer to deletion and repetition errors as shift errors. These types of synchronization error define a channel that has been studied extensively by information theorists~\cite{gallager1961sequential,dobrushin1967shannon,ullman1967capabilities,diggavi2001transmission,kavcic2004insertion,diggavi2007capacity,mitzenmacher2009survey}. There is no closed form expression for the capacity of this insertion/repetition and deletion channel, but standard linear codes are known to be far from optimal. For example, the rate penalty for correcting a single shift error is logarithmic in the block length, but the optimal linear code has rate $1/2$~\cite{abdel2010correcting}.

% Synchronization errors pose interesting challenges to information and coding theorists. In particular, deletion channels have been studied in Information Theory since the 60's~\cite{gallager1961sequential,dobrushin1967shannon,ullman1967capabilities,diggavi2001transmission,kavcic2004insertion,diggavi2007capacity,mitzenmacher2009survey}, and the capacity of these channels remains unknown. There is no closed-form expression for the capacity, nor is there an efficient algorithmic means to numerically compute the capacity. 

% In this work, we study a new computer memory technology, namely racetrack memory, which is an example of deletion and insertion channels. Racetrack memory, a non-volatile memory that is engineered to provide both high density and fast read/write speed, is one of several emerging technologies that aim to replace conventional memories such as DRAM and Flash~\cite{mittalsurvey,thomas2011racetrack,sun2013cross}. It stores data in tape-like tracks and uses current injection to {\it shift} magnetic domains that store data bits on these tracks. In this technology, a deletion occurs when the injected current is larger than expected thus one or more domains are skipped. A repetition occurs when the injected current is smaller than expected and the domain under the port does not change, and we read the same bit two or more times. Broadly speaking, we refer to deletion and repetition errors as shift errors.

% This paper describes codes that correct deletions and repetitions in racetrack memory by separating the tasks of error detection and error correction. By organizing in this way, we make it extremely fast to read out data in the typical case, in which no error occurs. Detection is accomplished by introducing delimiter bits that identify when an error has occurred, as well as the error type. Correction is accomplished by a class of graph based codes, known as Varshamov-Tenengolts codes.

% We model the racetrack memory by limiting the number of shift errors that can happen close to each other. In particular, we allow for a maximum two shift (deletion or insertion) errors every $m+3$ shift operations. This model is a generalization of the one introduced in~\cite{liu2010codes} for deletion and insertion channels with segmented errors in which one shift error could happen per segment (a segment is a fixed number of input bits). Moreover in~\cite{liu2010codes}, authors assume either deletion errors or insertion errors but not a mixture of the two may occur in the channel; we impose no such constraint in our work.

% Our goal is to develop a code for this technology that meets that physical constraints of the technology and is deemed practical by computer architects. To that end, our code needs to have low implementation complexity and the corresponding encoding and decoding circuits should have low power consumption. 

There is some prior work in the computer architecture literature that seeks to handle shift errors by introducing extra read/write ports. The HiFi scheme presented in~\cite{HiFi} requires at least two extra reads and one extra write to access a stored bit. When an error is detected, it is corrected by reversing the current injection and reading the memory again. The extra read/write operations and the need for additional hardware limit the attractiveness of this solution and diminish the appeal of racetrack memory.

We propose an alternative solution, based on codes that detect and correct shift errors. The codes are easy to implement, and the circuits for encoding and decoding consume little power. Our coding solution does not require additional hardware, and it does not introduce additional reads or writes to memory.

Section~\ref{Section:Practical} describes a product code that can detect and correct up to two shift errors every $m+3$ shift operations in racetrack memory. The product structure makes it possible to decouple error detection from error correction, so that in the common case of no shift error, the access to stored data is fast. We detect up to two shift errors by combining Varshamov-Tenengolts (VT) codes~\cite{VTCodes} with blocks of delimiter bits. Our product construction extends the utility of VT codes, which are limited to correcting single shift errors, and we also provide a low complexity construction for these codes. The inner code detects up to two shift errors within a single track, and is able to correct one. The outer code connects data stored on different tracks, and makes it possible to correct two shift errors.

% We introduce a product code that can detect and correct up to two shift errors every $m+3$ shift operations in racetrack memory. An interesting objective for computer architects is to make the common case in which no error happens fast and efficient. To that end, it helps if one could decouple error detection from error correction. In order to detect up to two shift errors, we use Varshamov-Tenengolts (VT) codes~\cite{VTCodes} enhanced by a number of helper bits that we refer to as {\it delimiter bits}. We note that VT codes are not inherently capable of detecting more than a single shift error. Moreover, we introduce a low complexity construction algorithm for these codes.

% Single shift errors are corrected using the VT codes; beyond that we use the spatial diversity in racetrack memory and we deploy an outer-code across multiple tracks. In other words, within a single track, we can detect up to two shift errors and correct one and using an outer-code across multiple tracks, we can correct two shift errors as well. 

% In the Computer Architecture literature there is some prior work on racetrack memory, including handling shift errors by adding extra read/write ports~\cite{HiFi}. Reading a stored data bit from racetrack memory in the HiFi scheme~\cite{HiFi} is accompanied by at least two extra reads and one extra write. When an error is detected, the correction is done by reversing the current injection and reading the memory again. Adding extra hardware and read/write operations limits the attractiveness of racetrack technology. Compared to the prior work, our code handles shift errors at a low cost. Our code does not require any additional hardware and does not introduce extra reads or writes to the memory. Thus, our work improves upon storage rate, error correction cost, and hardware cost, and lowers the barrier for adopting racetrack in computer systems.

% The rest of the paper is organized as follows. In Section~\ref{Section:Racetrack}, we provide a brief background for racetrack memory and we introduce our error model. In Section~\ref{Section:Main}, we present our main result and characterize the achievable zero-error rate of our proposed code. Section~\ref{Section:Practical} introduces our code. Finally, Section~\ref{Section:Conclusion} concludes the paper and discussed future directions.

==> Submission ISIT 2017/Linear.tex <==
For Racetrack memory, one may wonder how well linear codes can perform. In fact from~\cite{}, we know that any linear code that can correct a deletion or a repetition has a storage rate less than or equal to $1/2$. We show that a very simple code can achieve arbitrary close to what is theoretically possible from linear codes.

\noindent {\bf Encoding}: The encoding is simply performed by writing each bit twice in the memory. Suppose $m=1k+3$, if the input data bits are denoted by $d_1,d_2,\ldots,d_k$, then we write the following $m$ bits on the memory:
\begin{align}
\underbrace{d_1 d_1 d_2 d_2 \ldots d_k d_k}_{\text{repetition~code}}\underbrace{100}_{\text{delimiter}}.
\end{align} 

\noindent {\bf Decoding}: Suppose using the delimiter bits we identify a deletion. Then, we must observe an odd number of $0$'s (or $1$'s) in the first $m-4$ bits. Add a single $0$ (or $1$) to this odd number of $0$'s (or $1$'s). Now, bits $b_1, b_3, b_5, \ldots, b_{m-4}$ are the stored data bits.

\noindent {\bf Performance}: The storage rate for this linear code, defined as the number of data bits stored in $m$ bits of the memory, is given by
\begin{align}
R_{\text{repetition}}\left( m \right) \overset{\triangle}= \frac{k}{\underbrace{2k+3}_{=~m}} \overset{m \rightarrow \infty}\rightarrow \frac{1}{2}.
\end{align}

In other words, using linear codes we have at least 100$\%$ overhead, \emph{i.e.} $k$ data bits are mapped to a minimum of $2k$ bits on the memory.

==> Submission ISIT 2017/Main.tex <==
In this section, we present our main contribution. First, we need the following definition.

\begin{definition}
If any $k$ input data bits can be mapped to some $m$-bit codeword such that the $k$ data bits can be recovered error-free under the assumptions of Section~\ref{Section:ErrorModel}, we say a zero-error rate of $k/m$ is achievable.
\end{definition}

\begin{theorem}
\label{THM:Main}
For racetrack memory with the error model defined in Section~\ref{Section:Racetrack} and with $r$ parallel tracks, we can achieve a zero-error rate of
\begin{align}
R_{0}\left( \ell, r \right) = \frac{r-1}{r} \times \frac{2^\ell - \ell - 1}{2^\ell+6}, \qquad \ell \in \mathbb{Z}^+,
\end{align}
where $k = 2^\ell - \ell - 1$ is the number of input data bits that are mapped to $m = 2^\ell+6$ magnetic domains on the memory.
\end{theorem}

Our code has three main components in two dimension. First dimension is within a single track where we use Varshamov-Tenengolts codes to store data. These codes are able to correct single shift errors. However, Varshamov-Tenengolts codes are not capable of detecting or correcting two shift errors. We enhance these codes by appending some helper bits that we refer to as {\it delimiter bits} which allow for double-shift-error detection per track. The role of the delimiter bits is to convert racetrack to a traditional deletion/insertion channel. The second dimension is across the $r$ tracks where we deploy a single parity-check code to correct double shift errors. The challenging part is to detect two shift errors and correct one. We use a simple outer code to correct two shift errors. 

% Imagine storing data in tracks. When we access data stored in a particular track, the common case is that we encounter single shift errors, and we can recover the data. Occasionally we detect two shift errors and then we have to go read some more data. This is a lot like 2D DRAM and we might make this connection.

% Also, we are enabling a class of coding solutions - Theorem 1 is a representative but other product codes are possible. What is important is the detection capability.

The rest of the paper is dedicated to the proof of Theorem~\ref{THM:Main}. We also note that $R_{0}\left( \ell, r \right) \rightarrow 1$ as $\ell,r \rightarrow \infty$. As an example, consider $\ell = 6$ (\emph{i.e.} $57$ input data bits) and $r = 8$. Then, we have $R_{0}\left( 6, 8 \right) = 0.7125$.


==> Submission ISIT 2017/Practical.tex <==
In this section, we introduce our code for racetrack memory and we prove Theorem~\ref{THM:Main}. We start with a single track and we devise a code that can correct a single shift error and detect up to two shift errors every $m+3$ shifts. We then show how to correct two shift errors using an outer code that takes advantage of the spatial diversity in racetrack memory. 

\begin{table*}[t]
\begin{center}
\begin{tabular}{|M|M|M|M|M|M|L|K|}
\hline
\multicolumn{7}{|c|}{Observation} & {\multirow{2}{*}{Decision}} \\
\cline{1-7}

position $m-5$ & position $m-4$ & position $m-3$ & position $m-2$ & position $m-1$ & position $m$ & Checksum {\bf mod~} $n+1$ & \\ \hline
1      &  1    &  0     & 0      &  {\sf X} &  {\sf X}  & =~0                 &  no error                   \\ \hline \rowcolor{Gray}
1      &  1    &  0     & 0      &  {\sf X} &  {\sf X}  & $\neq$~0            &  1 del. and 1 rep.: {\bf erasure}  \\ \hline 
1      &  0    &  0     & 0      &  {\sf X}  &  {\sf X}   & {\sf X}           &  1 deletion error           \\ \hline
{\sf X} &  1    &  1     & 0      &  0     &  {\sf X}   & {\sf X}             &  1 repetition error         \\ \hline 
0      &  0    &  0     & 0      &  {\sf X}     &  {\sf X}   & {\sf X}        &  2 deletion errors: {\bf erasure}         \\ \hline
{\sf X}      &  {\sf X}    &  1     & 1      &  0     &  0   & {\sf X}        &  2 repetition errors: {\bf erasure}       \\ \hline
\end{tabular}
\vspace{2mm}
\caption{Resulting observations in positions $m-2$, $m-1$ and $m$ for all possible error combinations and ${\sf X}$ indicates an irrelevant entry.\label{Table:Syndrom}}
% 
\end{center}
\vspace{-6mm}
\end{table*}


%\multicolumn{1}{|L|}{no error}                                 & 1      &  1    &  0     & 0      &  0     &  0   & =~0    \\ \hline
%\multicolumn{1}{|L|}{$1$ deletion}                             & 1      &  0    &  0     & 0      &  {\sf X}  &  {\sf X}   & {\sf X}    \\ \hline
%\multicolumn{1}{|L|}{$1$ repetition}                           & {\sf X} &  1    &  1     & 0      &  0     &  {\sf X}   & {\sf X}    \\ \hline 
%\multicolumn{1}{|L|}{$2$ deletions}                            & 0      &  0    &  0     & 0      &  {\sf X}     &  {\sf X}   & {\sf X}    \\ \hline
%\multicolumn{1}{|L|}{$2$ repetitions}                          & {\sf X}      &  {\sf X}    &  1     & 1      &  0     &  0   & {\sf X}    \\ \hline
%\multicolumn{1}{|L|}{$1$-del. $1$-rep. data correct}           & 1      &  1    &  0     & 0      &  0     &  0   & =~0    \\ \hline
%\multicolumn{1}{|L|}{$1$-del. $1$-rep. data wrong}             & 1      &  1    &  0     & 0      &  0     &  0   & $\neq$~0    \\ \hline


% \subsection{Single Track}
% \label{Section:SingleTrack}

% On a single track, we encode $k = 2^\ell - \ell - 1$ data bits into an {\it extended codeword} of length $m = 2^\ell+6$ which consists of a Varshamov-Tenengolts code (defined below) of length $n = m-6$ followed by six helper bits that we refer to as delimiter bits. 

On a single track, we encode the data bits into an {\it extended codeword} of length $m$ which consists of a Varshamov-Tenengolts code (defined below) of length $n = m-6$ followed by six helper bits that we refer to as delimiter bits.

\begin{definition}
The Varshamov-Tenengolts code $VT\left( n \right)$ is the set of all binary strings $\left( c_1, c_2, \ldots, c_n \right)$ satisfying
\begin{align}
\label{eq:VTCondition}
\sum_{i=1}^n{ic_i} \overset{\mathbf{mod}~n+1}\equiv 0, 
\end{align}
where the sum is evaluated as an ordinary rational integer\footnote{Technically speaking, our definition is a specific instance of VT codes. In general, VT codes satisfy $\sum_{i=1}^n{ic_i} \overset{\mathbf{mod}~n+1}\equiv a$, and we used $a=0$.}.
\end{definition}

\begin{remark}
VT codes were introduced in~\cite{VTCodes} to correct errors on a Z-channel. It follows from (\ref{eq:VTCondition}) that these codes are nonlinear over the binary field.
% We note that VT codes were introduced in~\cite{VTCodes} for correcting errors on a Z-Channel. These codes are nonlinear due to (\ref{eq:VTCondition}). 
\end{remark}

\noindent {\bf Encoding:} It is possible to construct $VT\left( n \right)$ codes for any $n$, but to maximize the speed of encoding and decoding we choose $n = 2^\ell$ and $k = n-\ell-1$, because when $n+1 = 2^\ell + 1$ the necessary modular arithmetic can be executed more efficiently (see~\cite{piestrak1994design}). The encoding algorithm is described below.
% Suppose $n = 2^\ell$ and $k = n-\ell-1$. We encode $k$ data bits $d_1,d_2,\ldots,d_k$ into a codeword $\mathbf{c}$ of size $n$ such that it satisfies (\ref{eq:VTCondition}). We introduce the following construction algorithm that can be easily implemented\footnote{We can construct $VT\left( n \right)$ codes for any $n$; however, to provide fast and efficient encoding and decoding, we focus on powers of two, \emph{i.e.} $n = 2^\ell$. The reason is that our encoding and decoding require calculating modulo $n+1$ operation, and we know that modulo operation can be performed more efficiently~\cite{piestrak1994design} if $n+1$ is equal to $2^\ell+1$.}.
% \noindent\makebox[\linewidth]{\rule{\columnwidth}{0.8pt}}
\vspace{-2mm}
\begin{framed}
\begin{enumerate}[leftmargin=0.3cm]
\item Start with a zero-vector $\mathbf{c}$ of length $n = 2^\ell$.

\item Set positions that are not powers of two to data bits (there are $k = n-\ell-1$ such positions).

\item Set $s$ to be the minimum value that needs to be added to the checksum $\sum_{i=1}^n{ic_i}$ to make it equal to $0$ modulo $n+1$.

\item Set the $\ell+1$ positions that are powers of two to the binary expansion (of length $\ell+1$) of $s$. Start from $c_1$ and set it to the least significant bit of the binary expansion of $s$, and move all the way to $c_n$ and set it to the most significant bit of the binary expansion of $s$.
\end{enumerate}
\end{framed}
\vspace{-2mm}
%\noindent\makebox[\linewidth]{\rule{\columnwidth}{0.8pt}}
It is straightforward to verify that the resulting codeword satisfies (\ref{eq:VTCondition}). We know that in step $3$ we have $0 \leq s \leq n$. Since $n = 2^\ell$, the binary expansion of $s$ is at most $\ell+1$ bits long. 

After encoding the $k$ data bits into a codeword $\mathbf{c}$ of size $n$, we append six delimiter bits to create the \textit{extended codeword} of length $m = n + 6$ that we write to the memory. The six delimiter bits are fixed and equal to $\mathbf{110000}$.

In the remainder of this section, we show that the extended codeword introduced above can correct a single shift error and detect up to two shift errors every $m+3$ shifts. Then, we show how we can correct two shift errors. We present our argument in five steps. In steps~1 and~2, we show that VT codes are capable of correcting a single shift error. Step~3 shows how we can detect up to two shift errors and takes into account the fact that the memory controller is always going to provide the desired number of bits, regardless of whether an error occurs. Step~4 show how to correct a single shift error using our extended codeword. Finally, step~5 incorporates spatial diversity to correct two shift errors.

\vspace{1mm}
\noindent{{\bf Step~1: VT codes are single-deletion-error correcting codes.}} Consider two binary strings $\mathbf{x} = x_1,x_2,\ldots,x_{n}$ and $\mathbf{y} = y_1,y_2,\ldots,y_{n}$. Let $D_{-1}\left( \mathbf{x} \right)$ and $D_{-1}\left( \mathbf{y} \right)$ denote the set of all the binary strings of length $n-1$ that result from a single deletion in $\mathbf{x}$ and $\mathbf{y}$ respectively. If we wish to use these two strings to store different values in a single-deletion channel, we need
\begin{align}
\label{Eq:CodeRequirement}
D_{-1}\left( \mathbf{x} \right) \cap D_{-1}\left( \mathbf{y} \right) = \emptyset.
\end{align}

The following lemma shows that VT codes are single-deletion-error correcting codes.

\begin{lemma}[\cite{levenshtein1966binary,levenshtein1965binary}]
\label{Lemma:VTGraphBased}
Any two binary strings $\mathbf{x}, \mathbf{y} \in VT\left( n \right)$, satisfy (\ref{Eq:CodeRequirement}).
%\begin{align}
%D_{-1}\left( \mathbf{x} \right) \cap D_{-1}\left( \mathbf{y} \right) = \emptyset.
%\end{align}
\end{lemma}

For completeness, we present the proof of Lemma~\ref{Lemma:VTGraphBased} in Appendix~\ref{Appendix:AlgoDescription}.

\vspace{1mm}
\noindent{{\bf Step~2:  VT codes are single-insertion-error correcting codes.}} Note that a single-insertion-error correcting code is a single-repetition-error correcting code as well. Similar to what we described above, let $D_{+1}\left( \mathbf{x} \right)$ denote the set of all the binary strings of length $n+1$ that result from a single insertion in $\mathbf{x}$. We have the following result that shows the Varshamov-Tenengolts codes can be used for single-insertion-error-correction as well as single-deletion-error-correction.
\begin{lemma}
\label{Lemma:DeletionandInsertion}
If for two binary strings of length $n$ condition (\ref{Eq:CodeRequirement}) is satisfied, then we have
\begin{align}
\label{Eq:InsertionConstraint}
D_{+1}\left( \mathbf{x} \right) \cap D_{+1}\left( \mathbf{y} \right) = \emptyset.
\end{align}
In other words, a single-deletion-error correcting code is a single-insertion-error correcting code.
\end{lemma}
\begin{proof}
Suppose two binary strings $\mathbf{x}$ and $\mathbf{y}$ of length $n$ satisfy (\ref{Eq:CodeRequirement}) but not (\ref{Eq:InsertionConstraint}). Suppose inserting $x^\prime$ in position $i$ of $\mathbf{x}$ and $y^\prime$ in position $j$ of $\mathbf{y}$ results in the same sequence of length $n+1$. Without loss of generality, we assume $i \leq j$. This implies that deleting $x_{j-1}$ and $y_{i}$ from $\mathbf{x}$ and $\mathbf{y}$ respectively, would result in the same sequence of length $n-1$. This contradicts (\ref{Eq:CodeRequirement}), thus proving the lemma.
\end{proof}

\vspace{1mm}
\noindent{{\bf Step~3: Our extended codeword can detect up to two shift errors.}} In this step, we show that using the six delimiter bits and the checksum condition of (\ref{eq:VTCondition}), we can detect up to two shift errors. Consider $m$ consecutive magnetic domains in racetrack memory. If no error happens, we need $m-1$ shifts to access and read the $m$ bits stored in these $m$ domains. We summarize the resulting observations in positions $m-5,m-4,\ldots,m$ for all possible error combinations in Table~\ref{Table:Syndrom}. In Appendix~\ref{Appendix:Table}, we explain how Table~\ref{Table:Syndrom} is obtained.

\begin{figure}[t]
\centering
% height = 5.5cm
\includegraphics[height = 6cm]{FiguresPDF/OuterCode-Diversity.pdf}
\caption{Using an outer code on top of the code presented in Section~\ref{Section:Practical} allows us to correct two shift errors.\label{Fig:OuterCode}}
\vspace{-4mm}
\end{figure}


The most interesting case is when a combination of a deletion error and a repetition error takes place prior to the delimiter bits. In this case, we observe the delimiter bits as the error-free case, \emph{i.e.} $110000$. To detect such errors, we have the following result for VT codes.
\begin{lemma}
\label{Lemma:combination}
For any two binary strings  $\mathbf{x}, \mathbf{y} \in VT\left( n \right)$, $\mathbf{y}$ cannot be obtained from $\mathbf{x}$ by a deletion followed by an insertion (or by an insertion followed by a deletion).
\end{lemma}

\begin{proof}
Suppose $\mathbf{x}^\prime \in D_{-1}\left( \mathbf{x} \right)$ and $\mathbf{y}^\prime \in D_{-1}\left( \mathbf{y} \right)$. If $\mathbf{y}$ can be obtained from $\mathbf{x}$ by a deletion followed by an insertion, then 
\begin{align}
D_{+1}\left( \mathbf{x}^\prime \right) \cap D_{+1}\left( \mathbf{y}^\prime \right) \neq \emptyset.
\end{align}
In other words, $\mathbf{x}^\prime$ and $\mathbf{x}^\prime$ do not satisfy (\ref{Eq:InsertionConstraint}) which in turn implies that $\mathbf{x}$ and $\mathbf{y}$ do not satisfy (\ref{Eq:CodeRequirement}). However, this contradicts Lemma~\ref{Lemma:VTGraphBased}. This contradiction proves the result. A similar argument can be used when an insertion is followed by a deletion. 
\end{proof}
Lemma~\ref{Lemma:combination} immediately results in the following observation.
\begin{corollary}
A combination of a deletion error and an insertion error on $\mathbf{x} \in VT\left( n \right)$ either results in $\mathbf{x}$ or in $\mathbf{y} \notin VT\left( n \right)$ (an invalid codeword).
\end{corollary}

The shaded row in Table~\ref{Table:Syndrom} corresponds to a combination of a deletion error and an insertion error that resulted in an invalid codeword.


\noindent{{\bf Step~4: Our extended codeword can correct a single shift error and decode the data.}} First, we need to understand how to recover data in the error-free case.

\noindent {\bf Error-free decoding:} If no error is detected using the delimiter bits and the checksum, the $k = n-\ell-1$ data bits are simply retrieved from the positions in $\mathbf{c}$ that are not powers of two, \emph{i.e.} positions $3,5,6,7,9,$ etc. So the only remaining task is to correct a shift error when it happens. 

\vspace{1mm}
\noindent {\bf Correcting a deletion error:} Deletion errors can be corrected using the elegant algorithm proposed by Levenshtein~\cite{levenshtein1966binary,levenshtein1965binary}. This algorithm is presented below, and we refer the reader to~\cite{Sloane} for a mathematical analysis.
% Deletion error correction can be done using the elegant algorithm proposed by Levenshtein~\cite{levenshtein1966binary,levenshtein1965binary} presented below. The mathematical explanation of how this algorithm is able to correct a deletion error can be found in~\cite{Sloane}.
%\noindent\makebox[\linewidth]{\rule{\columnwidth}{0.8pt}}
\begin{framed}
\begin{enumerate}[leftmargin=0.3cm]
\item Suppose a codeword $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ from $VT\left( n \right)$ is stored in racetrack memory, and we detect a single deletion, and we observe $\mathbf{c}^\prime =  \left( c^\prime_1, c^\prime_2, \ldots, c^\prime_{n-1} \right)$.

\item Set $\omega$ to be the Hamming weight (number of $1$'s) of $\mathbf{c}^\prime$.

\item Calculate the checksum $\sum_{i=1}^{n-1}ic^\prime_i$ and set $s$ to be the minimum amount that needs to be added to the checksum in order to make it $0~\textbf{mod}~n+1$.

\item If $s \leq \omega$, we restore the codeword by adding a $0$ immediately to the left of the rightmost $s$ $1$'s. Otherwise, we restore the codeword by adding a $1$ immediately to the right of the leftmost $\left( s-\omega-1 \right)$ $0$'s. 
\end{enumerate}
\end{framed}
% \noindent\makebox[\linewidth]{\rule{\columnwidth}{0.8pt}}

Using this algorithm, we reconstruct the correct codeword and recover the dataword as discussed for the error free case. Note that while the decoding algorithm corrects the codeword, it does not reveal where the deletion occurred. 

\vspace{1mm}
\noindent {\bf Correcting an insertion error:} From Lemma~\ref{Lemma:DeletionandInsertion}, we know that VT codes can correct an insertion. The corresponding Insertion Correction Algorithm is a modified version of the Deletion Correction Algorithm presented above and is omitted here due to space limitations.
%\begin{framed}
%\begin{enumerate}[leftmargin=0.3cm]
%\item Suppose a codeword $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ from $VT^\prime\left( n \right)$ is stored in racetrack memory, and we detect a single repetition. Suppose we observe $\mathbf{c}^\prime = \left( c^\prime_1, c^\prime_2, \ldots, c^\prime_{n+1} \right)$.
%
%\item Set $\omega$ to be the Hamming weight (number of $1$'s) of $\mathbf{c}^\prime$.
%
%\item Calculate the checksum $\sum_{i=1}^{n-1}ic^\prime_i$ and set $s$ to be the minimum amount that needs to be deducted from the checksum in order to make it $0~\textbf{mod}~n+1$.
%
%\item If $s \leq \omega$, we restore the codeword by removing a $0$ immediately to the left of the rightmost $s$ $1$'s. Otherwise,  we restore the codeword by removing a $1$ immediately to the right of the leftmost $\left( s-\omega \right)$ $0$'s.  
%\end{enumerate}
%\end{framed}

\vspace{1mm}
\noindent{{\bf Step~5: The outer code corrects two shift errors.}} Suppose we detect two shift errors and the data is erased as in Table~\ref{Table:Syndrom}. We can use an outer code to recover data in this case as illustrated in Fig.~\ref{Fig:OuterCode} where the outer code is a simple single parity code. We note that per track we can correct single shift errors and detect up to two shift errors.


==> Submission ISIT 2017/Prior.tex <==
There is a limited body of work for error correction in racetrack memory. HiFi~\cite{HiFi} addresses bit deletions in racetrack memory by adding pattern bits at both edges of each track as well as additional read and write ports. The main idea is to read the pattern in parallel with the data bits. If the pattern does not match what was expected, bits are shifted in the reverse direction and the memory is re-read to recover the bits correctly. In order to implement a code that can correct a single deletion, two additional ports (one read and one read/write port) need to be placed in each of the tracks. HiFi assumes a 2D structure for racetrack which allows the addition of extra ports. However, as we discussed in Section~\ref{Section:Racetrack}, racetrack memory achieves high levels of density through its 3D U-shaped geometry which is the preferred structure. In this 3D geometry, adding extra ports will be extremely challenging, if not impossible. As bits are shifted during consecutive reads, some of the pattern bits are ``shifted out'' of the track and virtually get deleted. Thus, for every shift in racetrack, one data bit and two pattern bits are read, while at the same time a new pattern bit is written. The main drawback of this implementation is that it adds substantial physical area and energy overheads because of the additional read and write ports and operations. We also need to emphasize that the placement of additional read and write ports are only feasible because prior work assumes a flat 2D structure for racetrack instead of a U-shaped 3D geometry.

Varshamov-Tenengolts codes have been used for deletion and insertion channels with segmented errors~\cite{liu2010codes} in which deletions {\it or} insertions (but not a mixture of two) could occur. This is a more restrictive model than racetrack memory in which deletions and insertions could both happen. Moreover, if we input $n$ bits to deletion and insertion channels with segmented errors, the output would be a sequence of length $n^\prime$ from which we can easily deduct the number of shift errors. Again, this differs from racetrack memory in which the memory controller is always going to provide the desired number of bits, $n$, regardless of whether an error occurs. Finally, codewords are found using exhaustive search for a given length and the (randomized) construction algorithm adds more overhead compared to our scheme. It is worth noting that the encoding and decoding of~\cite{liu2010codes} are not designed for implementation and introduce extra hardware and energy overheads.

% However, this idea requires the pattern bits to have at least the same length as the data bits as you need to read at least one extra bit for every data bit. Additionally, 


% There is a limited body of work for error correction in racetrack memory. An example is~\cite{HiFi} where the key is adding new hardware. More precisely, in order to detect and correct a shift error of size $i$, $i+1$ additional read/write ports are added. When dealing with single shift errors, every read requires two extra reads and two extra writes to the parity bits. Moreover, the correction is not carried out through coding, rather when an error is detected, a current in the reverse direction is injected to re-read the stored bits. Hence, this method introduces overhead to area, latency, and energy consumption of a racetrack memory design. However, increasing power consumption and latency through adding extra hardware and read/write operations limits the attractiveness of racetrack technology.

==> Submission ISIT 2017/Problem.tex <==
In this section we introduce racetrack memory and our error model.

\subsection{Racetrack Background}

Racetrack memory stores data in $r$ parallel tape-like tracks. Each data bit is stored in a magnetic domain and neighboring domains are separated by a domain wall as depicted in Fig.~\ref{Fig:Racetrack}. All read/write ports and the physical substrate are fixed in position, and as current is passed through the track, the domains pass by magnetic read/write ports positioned near the wire. 
\begin{figure}[t]
\centering
\includegraphics[height = 3.5cm]{FiguresPDF/Racetrack.pdf}
\caption{A single track with one read/write port. One bit is stored per domain and two neighboring domains are separated by a domain wall.\label{Fig:Racetrack}}
% \vspace{-4mm}
\end{figure}

Racetrack memory suffers from deletion and repetition errors. Bits are stored on a track and are accessed by injecting a current to shift them and place them under the read/write port. A \emph{shift} is therefore the injection of the current in order to place the next bit under the read/write port. If the injected current is larger than expected, then we might skip one or multiple magnetic domains resulting in {\it deletion errors}. On the other hand, if the injected current is smaller than expected, the port's position might not change and we might read the same bit twice. We refer to this error as a {\it repetition error}. We refer to deletion and repetition errors as ``shift errors.'' 

In deletion channels as studied in information theory, the size of the output is equal to the size of the input minus the number of deletions. However, in racetrack memory, the memory controller is always going to provide the desired number of bits, say $n$, regardless of whether an error occurs, so that an error determines which $n$ bits are provided. This is an important characteristic of racetrack memory, and a consequence is that we first need to determine whether an error has occurred.

There is a difference between a {\it repetition} and an {\it insertion}. An insertion means introducing a new bit in a string regardless of the value of its preceding bits. However, a repetition requires the new bit to be equal to the bit right before it. Thus, a repetition error is an instance of an insertion error.

Our goal is to devise a practical code that would allow reliable data recovery in the presence of shift errors in racetrack memory, and for that we need to define the error model.

\subsection{Error Model}
\label{Section:ErrorModel}

We make the following assumptions:
\begin{enumerate}

\item In each track and in every $m+3$ shifts (shift is defined above), at most {\bf two} shift errors may occur. 

\item When reading $r$ parallel tracks, in every $m+3$ shifts (per track), at most one track may have two shift errors.

\end{enumerate}

As we see later, if the second assumption is violated, then we can detect the errors but we will only be able to correctly decode the data on the tracks that have a single shift error. A more restrictive model for deletion and insertion channels with segmented errors was used in~\cite{liu2010codes} in which only one shift error could happen per segment (a segment is a fixed number of input bits). Moreover in~\cite{liu2010codes}, authors assume either deletion errors or insertion errors but not a mixture of the two may occur in the channel; we impose no such constraint.






==> Submission ISIT 2017/Problem_Old.tex <==
Racetrack memory consists of a number of read/write ports that are fixed in position and a number of ``tracks'' that store data. To pack more storage per unit surface area, the tracks are packed in a ``U-shape'' format as depicted in Fig.~\ref{}. For simplicity, we choose a 2-D representation as depicted in Fig.~\ref{}. This representation is only used to depict our coding strategy in the following sections. Racetrack memory promises many advantages over the existing technologies such as higher density and much faster access speed. However, in practice the access speed is much slower (up to a $1000\times$) than expected. This is due to the unique error model in Racetrack memory that cannot be simply addressed by ECCs. In what follows, we describe the error model for Racetrack memory.

We assume that each track can store a total of $n$ bits and we assume a total of $s$ tracks. To access a particular position $i_1$ in track $j$ from a current position $i_0$, a specific amount of current, ${\sf I}\left( i_0 \rightarrow i_1 \right)$, is injected in track $\ell$ where the magnitude and sign are determined by $i_0$ and $i_1$ as shown in Fig.~\ref{} (the farther you wish to travel in the track, the higher the magnitude). We refer to $\left| i_1 - i_0 \right|$ as the step size. Let function ${\sf P}\left( \ell \right)$ denote the true position of track $\ell$, and $\hat{{\sf P}}\left( \ell \right)$ denote the system's estimation of the position of track $\ell$, $\ell = 1,2,\ldots,s$. Ideally, we wish 
\begin{align}
{\sf P}\left( \ell \right) = \hat{{\sf P}}\left( \ell \right).
\end{align}
However, this is not always the case as depicted in Fig.~\ref{}. Due to manufacturing imperfections when ${\sf I}\left( i_0 \rightarrow i_1 \right)$ is applied to track $\ell$, we might have
\begin{align}
{\sf P}\left( \ell \right) = i_1 \neq \hat{{\sf P}}\left( \ell \right) = i_1^\prime.
\end{align}
If 
\begin{align}
{\sf P}\left( \ell \right) < \hat{{\sf P}}\left( \ell \right),
\end{align}
then a {\it repetition error} of length $\hat{{\sf P}}\left( \ell \right) - {\sf P}\left( \ell \right)$ has occurred; and if 
\begin{align}
{\sf P}\left( \ell \right) > \hat{{\sf P}}\left( \ell \right),
\end{align}
then a {\it deletion error} of length ${\sf P}\left( \ell \right) - \hat{{\sf P}}\left( \ell \right)$ has occurred. In general as $\left| i_1 - i_0 \right|$ increases, so does the probability of having a deletion or an insertion error. 

Our goal is to devise a coding strategy that would allow reliable data recovery in presence of deletion and repetition errors in Racetrack memory.

==> Submission ISIT 2017/Related.tex <==
Varshamov-Tenegolts codes have been used for deletion and insertion channels with segmented errors~\cite{liu2010codes} in which a number of deletions or insertions (but not a mixture of two) could occur. This is a more restrictive model than racetrack memory in which deletions and insertions could both happen. Moreover, if we input $n$ bits to deletion and insertion channels with segmented errors, the output would be a sequence of length $n^\prime$ from which we can easily deduct the number of shift errors. Again, this differs from racetrack memory in which the memory controller is always going to provide the desired number of bits, $n$, regardless of whether an error occurs.

Finally, codewords are found using exhaustive search for a given length and the (randomized) construction algorithm adds more overhead compared to our scheme. It is worth noting that the encoding and decoding of~\cite{liu2010codes} are not designed for implementation and introduce extra hardware and energy overheads.

==> Submission ISIT 2017/SingleDeletion.tex <==
We focus on a single track. We detect and correct a single deletion error every $m-1$ shifts or equivalently every $m$ bits. We first describe the encoding and decoding and then clarify the ideas through an example. We do detection and correction separately. The key is the correction and detection is done through a simple trick that we refer to as ``delimiter bits.'' 

\noindent {\bf Detection:} To detect a single deletion, we use the following format. We use bits $1,2,\ldots,m-2$ to store data and we set bits $m-1$ and $m$ to $1$ and $0$ respectively; bits $m+1,m+2,\ldots,2m-2$ to store data and we set bits $2m-1$ and $2m$ to $1$ and $0$ respectively and so on. Consider the first $m$ bits as depicted in Fig.~\ref{}. We refer to the ``$10$'' pattern in positions $m-1$ and $m$ as the delimiter bits. Now, if any of the first $m-1$ bits ($b_1,b_2,\ldots,b_{m-2}$ and $p_1$) gets deleted then once we read the data, in position $m-1$ we obtain a $0$. This indicates a single deletion in the first $m-1$ bits. On the other hand, if bit $m$ gets deleted, the first $m-1$ bits have been retrieved correctly and we delay the detection to the next $m$ bits.

\noindent {\bf Correction:} Consider two sequences of bits $\vec{b} = b_1,b_2,\ldots,b_{n}$ and $\vec{c} = c_1,c_2,\ldots,c_{n}$. In order to be able to use these two sequences to store different values in the memory, we need to be able to distinguish them even after a single deletion. In other words, if $b_i$ and $c_j$ are deleted $i,j \in \{ 1,2,\ldots, n \}$, then the resulting sequences should not be identical. If two bit sequences $\vec{b}$ and $\vec{c}$ can be confused with a single deletion, we refer to them as conflicting and denote it by $\vec{b} \sim \vec{c}$; and if cannot be confused with a single deletion, we refer to them as non-conflicting and denote it by $\vec{b} \nsim \vec{c}$. Therefore, our goal is to find the maximum number of sequences of length $n$ such that each pair is non-conflicting. This problem can be nicely defined and solved in graph theoretical terms.

Consider all $2^{n}$ sequences of length $n$. We create a conflict graph $N = \left( \mathcal{V}, \mathcal{E} \right)$, where $\mathcal{V}$ is the node set and $\mathcal{E} \subseteq \mathcal{V} \times \mathcal{V}$ is the edge set. Each node in this graph corresponds to a unique binary sequence of length $m-2$ ($\left| \mathcal{V} \right| = 2^n$). For simplicity label the nodes with numbers $0,1,2,\ldots,2^{n}-1$ and let node $i$ correspond to the binary expansion $i$. Now, $\left( i, j \right) \in \mathcal{E}$ if and only if the binary expansions of $i$ and $j$ are conflicting. In this graph, a set of non-conflicting sequences corresponds to an {\it independent set}; and the maximum number of sequences of length $n$ corresponds to the size of the {\it maximum independent set}. This problem is well studied and understood in graph theory and we can calculate the size of the maximum independent set for various values of $n$, $\left| \mathcal{I}^n_{\sf max} \right|$. We use the binary sequences corresponding to the nodes in the maximum independent set as our codewords.

A useful bound~\cite{} gives us
\begin{align}
\left| \mathcal{I}^n_{\sf max} \right| \geq \frac{2^n}{n+1}.
\end{align}
Thus, considering the delimiter bits, we guarantee a storage rate, $R_n$, such that
\begin{align}
\label{Eq:RateLowerBound}
R_n \geq \frac{n-\log_2\left( n+1 \right) - 2}{n}.
\end{align}
For instance, we have $R_{32} \geq 0.75$. We note that (\ref{Eq:RateLowerBound}) gives us a lower-bound and for finite values of $n$, the rate is in fact better than the lower-bound. Moreover, we note that $\lim_{n \rightarrow \infty} R_n = 1$.

\noindent {\bf Encoding:} For a fixed $n$, we have $\left| \mathcal{I}^n_{\sf max} \right|$ non-conflicting sequences and thus, we can store $\log_2\left| \mathcal{I}^n_{\sf max} \right|$ data bits using such sequences. Sort the nodes $v_i \in \mathcal{I}^n_{\sf max}$ according to their indices so that
\begin{align}
\mathcal{I}^n_{\sf max} = \left\{ \hat{v}_1, \hat{v}_2, \ldots, \hat{v}_{\mathcal{I}^n_{\sf max}} \right\}.
\end{align}
Now, a data sequence corresponding to a value $D$ between $0$ and $2^{\left| \mathcal{I}^n_{\sf max} \right|}$ is mapped to $\hat{v}_{\text{binary~exp.~of~}D}$. 


\noindent {\bf Decoding:} Using our delimiter sequence, we can detect a single deletion. If no deletion happens, and we obtain $\hat{v}_j$ then the stored data is simply $j$. However, if a single deletion happens, we need to identify which $\hat{v}_j$ was initially stored. Let $\mathcal{D}_{\hat{v}_j}$ denote the set of all sequences of length $n-1$ that result from a single deletion from $\hat{v}_j$. Based on our construction, we have
\begin{align}
\mathcal{D}_{\hat{v}_i} \cap \mathcal{D}_{\hat{v}_j} = \emptyset, \qquad \forall~i \neq j,~\hat{v}_i,\hat{v}_j \in \mathcal{I}^n_{\sf max}.
\end{align}
Thus, given a sequence of length $n-1$ resulting from a single deletion from $\hat{v}_j$, uniquely identifies $\hat{v}_j$. Once we have $\hat{v}_j$, we know the stored value. Note that in general, we do {\it not} have  $\left| \mathcal{D}_{\hat{v}_i} \right| = \left| \mathcal{D}_{\hat{v}_j} \right|$.

\noindent {\bf A Single-Deletion Code of length $n = 5$:} After deriving the maximum independent set for $n=5$, we have the following six codewords to use: 
\begin{align}
\hat{v}_1 &\rightarrow 00000, \nonumber \\
\hat{v}_2 &\rightarrow 00011, \nonumber \\
\hat{v}_3 &\rightarrow 01110, \nonumber \\
\hat{v}_4 &\rightarrow 10101, \nonumber \\
\hat{v}_5 &\rightarrow 11000, \nonumber \\
\hat{v}_6 &\rightarrow 11111. \nonumber 
\end{align} 
We note that there might be more than one maximum independent sets for each value of $n$. Note that a single deletion does not create any confusion between these cosewords. Moreover, note that $\mathcal{D}_{\hat{v}_1} = \left\{ 0000 \right\}$ and $\mathcal{D}_{\hat{v}_4} = \left\{ 0101, 1101,1001,1011,1010 \right\}$. Now, if we read out ``$0101$'' we know that we used codeword $\hat{v}_4 \rightarrow 10101$ and the stored data is $4$. Finally as mentioned before, we need to use the delimiter bits to store our data. So, if we want to store $2,4,$ and $5$ then on the memory we write:
$$\underbrace{00011}_{\hat{v}_2}\mathbf{10}\underbrace{10101}_{\hat{v}_4}\mathbf{10}\underbrace{11000}_{\hat{v}_5}\mathbf{10}.$$


==> Submission ISIT 2017/SingleDeletionConcept.tex <==
Our goal in this subsection is to show how one can use a graph-based code to correct a single deletion error. We first describe the key idea and present an example. We then formally define this code. We note that the idea of using graph-based codes to correct deletion errors has been previously used for communication systems~\cite{Sloane}. We assume that error detection is already performed using the delimiter bits introduced in the previous section. We denote binary strings with boldface letters, \emph{e.g.}, $\mathbf{x}$, and bits in these strings are denoted by lowercase letters, \emph{e.g.}, $x_1$. To label different binary strings, we use different boldface letters, \emph{e.g.}, $\mathbf{x}$ and $\mathbf{y}$. % , or we may use subscripts for the boldface letters, \emph{e.g.}, $\mathbf{x}_1$ and $\mathbf{x}_2$.

\noindent {\bf Key idea:} Consider two binary strings $\mathbf{x} = x_1,x_2,\ldots,x_{n}$ and $\mathbf{y} = y_1,y_2,\ldots,y_{n}$. In order to be able to use these two strings to store different values in racetrack memory, we need to be able to distinguish them even after a single deletion. In other words, if $x_i$ and $y_j$ are deleted for $i,j \in \{ 1,2,\ldots, n \}$, then the resulting binary strings should not be identical. If two binary strings $\mathbf{x}$ and $\mathbf{y}$ can be confused with a single deletion, we refer to them as {\it conflicting} with regards to deletion; if they cannot be confused with a single deletion, we refer to them as {\it non-conflicting} with regards to deletion. Consider the following set of binary strings.
\begin{align}
\label{Eq:CodewordsExample}
\left\{ \underbrace{00000}_{\mathbf{c}_0}, \underbrace{00011}_{\mathbf{c}_1}, \underbrace{01110}_{\mathbf{c}_2}, \underbrace{10101}_{\mathbf{c}_3}, \underbrace{11000}_{\mathbf{c}_4}, \underbrace{11111}_{\mathbf{c}_5} \right\}.
\end{align}

These six strings/codewords are pairwise non-conflicting. Let $D_{\mathbf{c}_j}$ denote the set of all strings of length $4$ that result from a single deletion in $\mathbf{c}_j$. In this example, $D_{\mathbf{c}_0} = \left\{ 0000 \right\}$ and $D_{\mathbf{c}_3} = \left\{ 0101, 1101,1001,1011,1010 \right\}$. Thus, if we read out ``$0101$'' we know that it refers to codeword $\mathbf{c}_3 = 10101$. 

Using the codewords of (\ref{Eq:CodewordsExample}), we can store six different values, say $0,1,\ldots,5$. So, if we want to store values $2,4,$ and $5$ to memory, the actual bits written to memory are:
\begin{align}
\label{Eq:CodeOnMemory}
\underbrace{01110}_{\mathbf{c}_2}\underbrace{\mathbf{100}}_{\text{delimiter}}\underbrace{11000}_{\mathbf{c}_4}\underbrace{\mathbf{100}}_{\text{delimiter}}\underbrace{11111}_{\mathbf{c}_5}\underbrace{\mathbf{100}}_{\text{delimiter}}.
\end{align}

\noindent {\bf Formal definition:} Consider all $2^{n}$ binary strings of length $n$. We create a conflict graph $N = \left( V, E \right)$, where $V$ is the node set and $E \subseteq V \times V$ is the edge set. Each node in this graph corresponds to a unique binary string of length $n$ ($\left| V \right| = 2^n$). For simplicity, label the nodes with numbers $0,1,2,\ldots,2^{n}-1$ and let node $i$ correspond to the binary expansion (of length $n$) of $i$ that we denote by $\mathbf{b}_i$. 

Now, $\left( i, j \right) \in E$ if and only if $\mathbf{b}_i$ and $\mathbf{b}_j$ are conflicting. In this graph, a set of non-conflicting strings corresponds to an {\it independent set}; the maximum number of strings of length $n$ corresponds to the size of the {\it maximum independent set}. For a given $n$, denote the maximum independent set by $I_n$. We use the binary strings corresponding to the nodes in the maximum independent set as our codewords. We note that the maximum independent set of a graph is not necessarily unique.

\noindent {\bf Encoding and decoding:} For a fixed $n$, we have $\left| I_n \right|$ non-conflicting strings and thus, we can store $\log_2\left| I_n \right|$ (for now assume this number is an integer) data bits using such strings. If $\mathbf{c}_i, \mathbf{c}_j \in I_n$ then $D_{\mathbf{c}_i} \neq D_{\mathbf{c}_j}$, thus decoding can be perofrmed by identifying from which codeword the observed sequence is obtained from.

The downside of encoding and decoding as described above is that you need to use a lookup table to find the right codeword. Using a lookup table is practical for short codewords but as the codeword length increases, the lookup table grows exponentially in size.

\begin{table*}[t!]
\begin{center}
\begin{tabular}{|K{\columnwidth}|K{\columnwidth}|N}
\hline
{\bf Encoding Algorithm}                                 & {\bf Example for $n=8,~\ell = 3$} &\\[10pt] \hline
{\bf Step~1}: Start with a zero-vector $\mathbf{c}$ of length $n = 2^\ell$.    &  $\mathbf{c} = c_1c_2\ldots c_8 = 00000000$ &\\[10pt] \hline
{\bf Step~2}: Set positions that are not powers of two to data bits.  & $\mathbf{d} = 1011~\rightarrow~\mathbf{c} = 00\underline{1}0\underline{011}0$ &\\[9pt] \hline
{\bf Step~3}: Calculate the checksum $\sum_{i=1}^n{ic_i}$.   & $\sum_{i=1}^n{ic_i} = 3 + 6 + 7 = 16$  &\\[9pt] \hline
{\bf Step~4}: Set $s$ to be the minimum value that needs to be added to the checksum to make it equal to $0$ modulo $n+1$.       &  $s=2$   &\\[20pt] \hline
{\bf Step~5}: Set the $\ell+1$ positions that are powers of two to the binary expansion (of length $\ell+1$) of $s$. Start from $c_1$ and set it to the least significant bit (LSB) of the binary expansion of $s$, and move all the way to $c_n$ and set it to the most significant bit (MSB) of the binary expansion of $s$.  & $s = \left( 0010 \right)_2~\rightarrow~c_1 = 0,~c_2 = 1,~c_4 = 0,~c_8 = 0 \newline \rightarrow~\mathbf{c} = \underline{01}1\underline{0}011\underline{0}$   &\\[30pt]\hline 
\end{tabular}
\vspace{2mm}
\caption{Encoding algorithm alongside an example for $n=8$.\label{Table:Encoding}}
\end{center}
\end{table*}

\begin{table*}[ht!]
% \large
\begin{center}
\begin{tabular}{|K{\columnwidth}|K{\columnwidth}|N}
\hline
{\bf Deletion Correction Algorithm}                                 & {\bf Example for $n=8,~\ell = 3$} &\\[10pt] \hline
{\bf Step~1}: Suppose a codeword $\mathbf{c} = \left( c_1, c_2, \ldots, c_n \right)$ from $VT\left( n \right)$ is stored in racetrack memory, and using the delimiter bits, we identify a single deletion, and we observe $\mathbf{c}^\prime =  \left( c^\prime_1, c^\prime_2, \ldots, c^\prime_{n-1} \right)$.    &  $\mathbf{c} = 011001\underline{1}0~\rightarrow~\mathbf{c}^\prime = 0110010$ &\\[30pt] \hline
{\bf Step~2}: Set $\omega$ to be the Hamming weight (number of $1$'s) of $\mathbf{c}^\prime$.  & $\omega=3$ &\\[12pt] \hline
{\bf Step~3}: Calculate the checksum $\sum_{i=1}^{n-1}ic^\prime_i$. & $\sum_{i=1}^{7}ic^\prime_i = 11$ &\\[9pt] \hline
{\bf Step~4}: Set $s$ to be the minimum amount that needs to be added to the checksum in order to make it $0~\textbf{mod}~n+1$.  & $s = 7$ &\\[20pt] \hline
{\bf Step~5}: If $s \leq \omega$, we restore the codeword by adding a $0$ immediately to the left of the rightmost $s$ $1$'s. Otherwise, we restore the codeword by adding a $1$ immediately to the right of the leftmost $\left( s-\omega-1 \right)$ $0$'s.   & $e>\omega~\rightarrow~$restore the codeword by adding a $1$ immediately to the right of the leftmost $\left( s-\omega-1 \right) = 3$ zeros to arrive at the correct codeword: $01100\underline{1}10$.               &\\[30pt] \hline
\end{tabular}
\vspace{2mm}
\caption{Deletion Correction Algorithm alongside an example for $n=8$.\label{Table:Decoding}}
\end{center}
\end{table*}


We have the following result for the graph-based codes introduced in this section which proves that these codes can be used to correct a single insertion (and therefore, a single repetition) as well as a single deletion.
\begin{lemma}
\label{Lemma:DeletionandInsertion}
If two binary strings are non-conflicting with regards to deletion, then they are non-conflicting with regards to insertion.
\end{lemma}
\begin{proof}
Suppose two binary strings $\mathbf{x}$ and $\mathbf{y}$ of length $n$ are non-conflicting with regards to deletion but conflicting with respect to insertion. Suppose inserting $x^\prime$ in position $i$ of $\mathbf{x}$ and $y^\prime$ in position $j$ of $\mathbf{y}$ results in the same sequence of length $n+1$. Without loss of generality, we assume $i \leq j$. This implies that deleting $x_{j-1}$ and $y_{i}$ from $\mathbf{x}$ and $\mathbf{y}$ respectively, would result in the same sequence of length $n-1$. This contradicts the assumption that $\mathbf{x}$ and $\mathbf{y}$ are non-conflicting with regards to deletion, thus proving the lemma.
\end{proof}

It is also worth noting an important difference between the graph based codes and conventional error-correcting codes. In conventional ECCs, Hamming distance defines a sphere around each codeword and if this sphere has radius $t$, then their centers are codewords of a $\left(2t + 1\right)$-error-correcting code. Graph-based codes do not rely on Hamming distance but they rather rely on having disjoint sub-strings of length $n-1$ as denoted by $D_{{\mathbf{c}}_j}$ above. Unlike conventional ECCs where all spheres have equal radius, these disjoint sets associated with the graph-based codewords do not all have the same size as we saw for the codewords in (\ref{Eq:CodewordsExample}).

==> Submission ISIT 2017/Table.tex <==
In this appendix we describe how the combination of a VT code and six delimiter bits can be used to to identify two deletions, or a deletion and a repetition. The other cases appearing in Table~\ref{Table:Syndrom} can be derived using similar arguments.
% In this Appendix, we describe the rationale behind Table~\ref{Table:Syndrom}. We describe the scenarios in which either two deletions happen or a combination of a deletion and a repetition happens. The other cases can be derived using similar arguments. We remind the reader that we write an extended codeword on the memory which consists of a VT code and six delimiter bits.

\noindent {\bf Two deletions:} There are three cases to consider as listed below.
\begin{enumerate}

\item {\bf Two deletions in the VT code:} In  this case, in positions $m-5, m-4, m-3,$ and  $m-2$ we observe $0000$ and position $m-1$ corresponds to the first bit of the next extended codeword. In this case, we declare erasure and we use the outer-code to resolve this case.

\item {\bf Two deletions in the delimiter bits:} For this scenario, the VT code is unaffected. However, we will declare either one or two deletions as we cannot identify the location of these errors. In positions $m-5, m-4, m-3,$ and  $m-2$ we can observe three possibilities as described below and position $m-1$ corresponds to the first bit of the next extended codeword.
\begin{enumerate}

\item $0000$: Similar to the case when two deletions happen in the VT code, we declare an erasure. The VT code is not affected but since we cannot determine that the errors were within the delimiter bits, we cannot trust the checksum. We declare erasure and we use the outer-code to resolve this case.

\item $1000$: According to Table~\ref{Table:Syndrom}, we declare a single deletion. Again note that the VT code is not affected here. So even if we assume a single deletion, data can be reliably recovered. The second deletion error will be detected when we reach the next set of delimiter bits are obtained. We note that our assumption of at most two shift errors every $m+3$ shifts is needed to guarantee that the second shift error will be detected.

\item $1100$: According to Table~\ref{Table:Syndrom}, this is an error free case. Since the VT code is not affected here, data can be reliably recovered. However, if there was no error at all, positions $m-1$ and $m$ would correspond to the last two of the six delimiter bits. On the other hand, here positions $m-1$ and $m$ correspond to the first two bits of the next extended codeword and we deal with that when the next set of delimiter bits are obtained.

\end{enumerate} 

\item {\bf One deletion in the VT code and one deletion in the delimiter bits:} For this case, in positions $m-5, m-4, m-3,$ and  $m-2$ we can observe two possibilities as described below and position $m-1$ corresponds to the first bit of the next extended codeword.
\begin{enumerate}

\item $0000$: Similar to the case when two deletions happen in the VT code, we declare an erasure. The VT code only contains a single deletion but since we cannot determine this fact, we cannot trust the checksum. We use the outer-code to resolve this case.

\item $1000$: According to Table~\ref{Table:Syndrom}, we declare a single deletion. Since the VT code only contains a single shift error, data can be reliably recovered. 

\end{enumerate}

\end{enumerate}

\noindent {\bf One deletion and one repetition:} We discussed the case when one deletion and one repetition happen within the VT code in Step~3 of Section~\ref{Section:Practical}. Suppose one deletion happens in the VT code and one repetition in the delimiter bits. For this case, in positions $m-5, m-4, m-3,$ and  $m-2$ we can observe two possibilities as described below. The case in which one repetition happens in the VT code and one deletion in the delimiter bits can be explained similarly.
\begin{enumerate}

\item $1000$: According to Table~\ref{Table:Syndrom}, we declare a single deletion. Since the VT code only contains a single shift error, data can be reliably recovered. 

\item $1100$: If the checksum is zero modulo $n+1$, we were lucky and the deletion followed by introducing the first bit of the delimiter bits in position $m-6$ resulted in the correct codeword. If the checksum is not zero modulo $n+1$, we declare erasure and we use the outer-code to resolve this case.
\end{enumerate}



==> Submission ISIT 2017/VTCodes.tex <==
In the previous subsection, we showed that it is possible to obtain codes that can correct a deletion error. The main drawback of naively using these graph-based codes is the issue of encoding and decoding which involves the use of a lookup table which is only practical for short codewords. In what follows, we impose a constraint on the graph-based codes introduced in Section~\ref{Section:Concept} that allows faster and more efficient encoding and decoding. The constraint we impose on the graph-based codes makes our code a Varshamov-Tenengolts (VT) code for which we introduce a new construction. 

\noindent {\bf Formal definition:} A Varshamov-Tenengolts code $VT\left( n \right)$ consists of all binary strings $\left( c_1, c_2, \ldots, c_n \right)$ satisfying
\begin{align}
\label{eq:VTCondition}
\sum_{i=1}^n{ic_i} \overset{\mathbf{mod}~n+1}\equiv 0, 
\end{align}
where the sum is evaluated as an ordinary rational integer.


Let's reconsider the example we provided in Section~\ref{Section:Concept} for $n=5$. We can pick a different set of six codewords compared to (\ref{Eq:CodewordsExample}) that correspond to an independent set and at the same time, satisfy (\ref{eq:VTCondition}):
\begin{align}
\label{Eq:VT5}
VT&\left( 5 \right) \\
& = \left\{00000,~10001,~01010,~11011,~11100,~00111\right\}. \nonumber
\end{align}
Note that the codewords in (\ref{Eq:CodewordsExample}) do not necessarily satisfy the imposed constraint of (\ref{eq:VTCondition}). We have the following result for the Varshamov-Tenegolts codes.
\begin{theorem}
\label{THM:VT}
VT codes correspond to an independent set of the graph $N = \left( V, E \right)$ introduced in the previous subsection.
\end{theorem}

To prove Theorem~\ref{THM:VT}, it suffices to show that we can uniquely identify the codeword after a single deletion. We do so later in this section when we discuss decoding VT codes.

In the rest of this section, we provide the answer the following questions:
\begin{enumerate}

\item How to encode data using Varshamov-Tenengolts codes?

\item How to decode data and correct an error if it happens?

\end{enumerate}

With an eye for implementation, we introduce a new construction algorithm for Varshamov-Tenengolts codes. We can construct $VT\left( n \right)$ codes for any $n$; however, to provide fast and efficient encoding and decoding, we focus on powers of two, \emph{i.e.} $n = 2^\ell$. The reason is that our encoding and decoding require calculating modulo $n+1$ operation, and we know that modulo operation can be performed more efficiently~\cite{piestrak1994design} if $n+1$ is equal to $2^\ell+1$. Our code will correct one shift error every $m-1$ shifts where we assume a codeword of length $n$ and an extended codeword of length $m = n + 3$.

\noindent {\bf Encoding:} Suppose $n = 2^\ell$ and $k \overset{\triangle}= n-\ell-1$. We encode $k$ data bits $d_1,d_2,\ldots,d_k$ into a codeword $\mathbf{c}$ of size $n$ such that it satisfies (\ref{eq:VTCondition}).

We present the encoding algorithm and an example for $n=8$ in Table~\ref{Table:Encoding}. For this example, $\ell=3$ and we encode $k = n - \ell -1 = 4$ data bits ($1011$) into a codeword of length $n=8$. The encoding algorithm creates $\ell + 1$ check bits to ensure that (\ref{eq:VTCondition}) holds. We index bit positions in a codeword from $1$ to $n$ (rather than $0$ to $n-1$). It is worth noting that for this small example of length $n=8$, our code has the same rate as a linear code. However, as $n$ grows larger, our code quickly outperforms any linear code.

After encoding the $k$ data bits into a codeword $\mathbf{c}$ of size $n$, we append the delimiter bits to create the extended codeword of length $m = n + 3$ that we write to the memory. We can calculate the code rate as:
\begin{align}
& R_{\text{VT}}\left( m \right) = \frac{m - \log_2(m-3) - 4}{m} \overset{m \rightarrow \infty}\rightarrow 1.
\end{align}

\vspace{1mm}
\noindent {\bf Error-free decoding:} If no error is detected using the delimiter bits, the $k = n-\ell-1$ data bits are simply retrieved from the positions in $\mathbf{c}$ that are not powers of two, \emph{i.e.} positions $3,5,6,7,9,$ etc. So the only remaining task is to correct a shift error when it happens. 

\vspace{1mm}
\noindent {\bf Correcting a deletion error:} Deletion error correction can be done using the elegant algorithm proposed by Levenshtein~\cite{levenshtein1966binary,levenshtein1965binary} which we present in Table~\ref{Table:Decoding} alongside an example for $n=8$. The mathematical explanation of how this algorithm is able to correct a deletion error can be found in~\cite{Sloane}.

Using the decoding algorithm, we reconstruct the correct codeword and recover the dataword as discussed for the error free case. It is worth mentioning that while the decoding algorithm corrects the codeword, it does not reveal where the deletion occurred. In fact, if either of the $1$'s in positions $6$ or $7$ was deleted, the algorithm would have behaved exactly the same way.

\vspace{1mm}
\noindent {\bf Correcting an insertion error:} From Lemma~\ref{Lemma:DeletionandInsertion}, we know that VT codes can correct an insertion. The corresponding Insertion Correction Algorithm is very similar to the Deletion Correction Algorithm and follows the same logic. Due to space limitations, we omit the Insertion Correction Algorithm.


==> Submission ISIT 2017/VTCodes_Repetition.tex <==
Handling an insertion (and therefore a repetition) is very similar to handling a deletion and follows the same logic. We modify the Deletion Correction Algorithm to handle a repetition as given in Table~\ref{Table:RepDecoding}. Again, it is worth mentioning that while the algorithm corrects the codeword, it does not tell you where the repetition occurred.

==> VTCodes.tex <==
In the previous subsection, we showed that it is possible to obtain codes that can correct a deletion error. The main drawback of naively using these graph-based codes is the issue of encoding and decoding which involves the use of a lookup table which is only practical for short codewords. In what follows, we impose a constraint on the graph-based codes introduced in Section~\ref{Section:Concept} that allows faster and more efficient encoding and decoding. The constraint we impose on the graph-based codes makes our code a Varshamov-Tenengolts (VT) code for which we introduce a new construction. 

\noindent {\bf Formal definition:} A Varshamov-Tenengolts code $VT\left( n \right)$ consists of all binary strings $\left( c_1, c_2, \ldots, c_n \right)$ satisfying
\begin{align}
\label{eq:VTCondition}
\sum_{i=1}^n{ic_i} \overset{\mathbf{mod}~n+1}\equiv 0, 
\end{align}
where the sum is evaluated as an ordinary rational integer.


Let's reconsider the example we provided in Section~\ref{Section:Concept} for $n=5$. We can pick a different set of six codewords compared to (\ref{Eq:CodewordsExample}) that correspond to an independent set and at the same time, satisfy (\ref{eq:VTCondition}):
\begin{align}
\label{Eq:VT5}
VT&\left( 5 \right) \\
& = \left\{00000,~10001,~01010,~11011,~11100,~00111\right\}. \nonumber
\end{align}
Note that the codewords in (\ref{Eq:CodewordsExample}) do not necessarily satisfy the imposed constraint of (\ref{eq:VTCondition}). We have the following result for the Varshamov-Tenegolts codes.
\begin{theorem}
\label{THM:VT}
VT codes correspond to an independent set of the graph $N = \left( V, E \right)$ introduced in the previous subsection.
\end{theorem}

To prove Theorem~\ref{THM:VT}, it suffices to show that we can uniquely identify the codeword after a single deletion. We do so later in this section when we discuss decoding VT codes.

In the rest of this section, we provide the answer the following questions:
\begin{enumerate}

\item How to encode data using Varshamov-Tenengolts codes?

\item How to decode data and correct an error if it happens?

\end{enumerate}

With an eye for implementation, we introduce a new construction algorithm for Varshamov-Tenengolts codes. We can construct $VT\left( n \right)$ codes for any $n$; however, to provide fast and efficient encoding and decoding, we focus on powers of two, \emph{i.e.} $n = 2^\ell$. The reason is that our encoding and decoding require calculating modulo $n+1$ operation, and we know that modulo operation can be performed more efficiently~\cite{piestrak1994design} if $n+1$ is equal to $2^\ell+1$. Our code will correct one shift error every $m-1$ shifts where we assume a codeword of length $n$ and an extended codeword of length $m = n + 3$.

\noindent {\bf Encoding:} Suppose $n = 2^\ell$ and $k \overset{\triangle}= n-\ell-1$. We encode $k$ data bits $d_1,d_2,\ldots,d_k$ into a codeword $\mathbf{c}$ of size $n$ such that it satisfies (\ref{eq:VTCondition}).

We present the encoding algorithm and an example for $n=8$ in Table~\ref{Table:Encoding}. For this example, $\ell=3$ and we encode $k = n - \ell -1 = 4$ data bits ($1011$) into a codeword of length $n=8$. The encoding algorithm creates $\ell + 1$ check bits to ensure that (\ref{eq:VTCondition}) holds. We index bit positions in a codeword from $1$ to $n$ (rather than $0$ to $n-1$). It is worth noting that for this small example of length $n=8$, our code has the same rate as a linear code. However, as $n$ grows larger, our code quickly outperforms any linear code.

After encoding the $k$ data bits into a codeword $\mathbf{c}$ of size $n$, we append the delimiter bits to create the extended codeword of length $m = n + 3$ that we write to the memory. We can calculate the code rate as:
\begin{align}
& R_{\text{VT}}\left( m \right) = \frac{m - \log_2(m-3) - 4}{m} \overset{m \rightarrow \infty}\rightarrow 1.
\end{align}

\vspace{1mm}
\noindent {\bf Error-free decoding:} If no error is detected using the delimiter bits, the $k = n-\ell-1$ data bits are simply retrieved from the positions in $\mathbf{c}$ that are not powers of two, \emph{i.e.} positions $3,5,6,7,9,$ etc. So the only remaining task is to correct a shift error when it happens. 

\vspace{1mm}
\noindent {\bf Correcting a deletion error:} Deletion error correction can be done using the elegant algorithm proposed by Levenshtein~\cite{levenshtein1966binary,levenshtein1965binary} which we present in Table~\ref{Table:Decoding} alongside an example for $n=8$. The mathematical explanation of how this algorithm is able to correct a deletion error can be found in~\cite{Sloane}.

Using the decoding algorithm, we reconstruct the correct codeword and recover the dataword as discussed for the error free case. It is worth mentioning that while the decoding algorithm corrects the codeword, it does not reveal where the deletion occurred. In fact, if either of the $1$'s in positions $6$ or $7$ was deleted, the algorithm would have behaved exactly the same way.

\vspace{1mm}
\noindent {\bf Correcting an insertion error:} From Lemma~\ref{Lemma:DeletionandInsertion}, we know that VT codes can correct an insertion. The corresponding Insertion Correction Algorithm is very similar to the Deletion Correction Algorithm and follows the same logic. Due to space limitations, we omit the Insertion Correction Algorithm.


==> VTCodes_Repetition.tex <==
Handling an insertion (and therefore a repetition) is very similar to handling a deletion and follows the same logic. We modify the Deletion Correction Algorithm to handle a repetition as given in Table~\ref{Table:RepDecoding}. Again, it is worth mentioning that while the algorithm corrects the codeword, it does not tell you where the repetition occurred.
